Universal characteristics of deep neural network loss surfaces from random matrix theory

This paper considers several aspects of random matrix universality in deep neural networks. Motivated by recent experimental work, we use universal properties of random matrices related to local statistics to derive practical implications for deep neural networks based on a realistic model of their Hessians. In particular we derive universal aspects of outliers in the spectra of deep neural networks and demonstrate the important role of random matrix local laws in popular pre-conditioning gradient descent algorithms. We also present insights into deep neural network loss surfaces from quite general arguments based on tools from statistical physics and random matrix theory.

==> almost-free.tex <==
%auto-ignore
\section{Spectra of noise models with local laws}
% \begin{lem}
% Let $\Lambda$ be the eigenvalues of a symmetric random matrix $X$ and CONDITION.
% Define the constant
% \begin{align}
%     q = \int d\mu_X(\lambda) |\lambda|.
% \end{align}
% Then for any real deterministic $c_N$
% \begin{align}
%     \E_{\Lambda}\exp\left(-iN^{-(1+\epsilon)}c_N\int \Tr|\Lambda|\right) = \exp\left(-iN^{-\epsilon} (q+o(1))c_N\right) + o(1)
% \end{align}
% where the $o(1)$ terms contain no dependence on the term $c_N$.
% \end{lem}
% \begin{proof}
%     Begin by defining $\delta = N^{-1}\Tr|\Lambda| - q$. We clearly have $|\E e^{-iN^{-\epsilon}c_N \delta}| \leq 1$. We will now establish a complimentary lower bound. 
% \end{proof}

% Given that $|\E e^{-iN^{-\epsilon}c_N \delta}| = 1 + o(1)$, we can certainly write \begin{align}
%     \E e^{-iN^{-\epsilon}c_N \delta} = e^{iN^{-\epsilon}c_N \sigma_N} + o(1)
% \end{align}
% for some real $\sigma_N$. Now formally differentiating both sides with respect to $c_N$, giving 
% \begin{align}
%      -iN^{-\epsilon}  \E[ \delta e^{-iN^{-\epsilon}c_N \delta}] &= -iN^{-\epsilon} \sigma_N e^{-iN^{-\epsilon}c_N \sigma_N}\notag\\
%      \implies |\E[ \delta e^{-iN^{-\epsilon}c_N \delta}]| &= |\sigma_N|
% \end{align}
% from which it follows that 
% \begin{align}
%     |\sigma_N| \leq \E |\delta| \leq \sqrt{\E\delta^2} = o(1)
% \end{align}
% where we have used Jensen's inequality and our assumption about the convergence of $N^{-1}\Tr|\Lambda|$. We have shown that $\sigma_N = o(1)$, which completes the proof. 

\begin{thm}\label{thm:nearly_free_addn}
    Let $X$ be an $N\times N$ real symmetric random matrix and let $D$ be an $N\times N$ symmetric matrix (deterministic or random). Let $\hat{\mu}_X, \hat{\mu}_{D}$ be the empirical spectral measures of the sequence of matrices $X, D$ and assume there exist deterministic limit measures $\mu_X, \mu_D$. Assume that $X$ obeys a local law (\ref{eq:local_law}) and the moment conditions of Theorem \ref{thm:que_gaussian} with measure $\mu_X$. Assume also the $\hat{\mu}_X$ concentrates in the sense that 
    \begin{align}\label{eq:concentration_condition}
        \P(W_1(\hat{\mu}_X, \mu_X) > \delta) \lesssim e^{-N^{\tau} f(\delta)}
    \end{align}
    where $\tau>0$ and $f$ is some positive increasing function.
    Then $H = X + D$ has a limiting spectral measure and it is given by the free convolution $\mu_X \boxplus \mu_D$.
\end{thm}
\begin{rem}
A condition like (\ref{eq:concentration_condition}) is required so that the Laplace method can be applied to the empirical measure $\hat{\mu}_X$. There are of course other ways to formulate such a condition.
\end{rem}
\begin{proof}
We shall denote use the notation \begin{align}
    G_H(z) = \frac{1}{N}\Tr (z - H)^{-1}.
\end{align}
Recall the supersymmetric approach to calculating the expected trace of the resolvent of a random matrix ensemble:
\begin{align}
    \E_H G_H(z) = \frac{1}{N}\frac{\partial}{\partial \j}\Bigg|_{\j=0} \mathbb{E}_H Z_H(\j)
\end{align}
where \begin{align}
    Z_H(\j) &= \frac{\det(z + \j - H)}{\det(z - H)} = \int d\Psi e^{-i\Tr AH} e^{i\Tr \Psi\Psi^{\dagger}J},\\
    A &= \phi\phi^{\dagger} + \chi\chi^{\dagger},\\
    J &= I_N \otimes \left(\begin{array}{cc} z & 0 \\ 0 & \j + z\end{array}\right),\\
    d\Psi &= \frac{d\phi d\phi^* d\chi d\chi^*}{-(2\pi)^N i},\\
    \Psi &= \left(\begin{array}{c} \phi \\ \chi \end{array}\right)
\end{align}
with $\phi\in\C^N$ and $\chi,\chi^*$ being $N$-long vectors of anti-commuting variables.
Independence of $X$ and $D$ gives
\begin{align}
    \E_H Z_H(\j) &= \int d\Psi e^{i\Tr \Psi\Psi^{\dagger}J} \E_{X,D} e^{-i\Tr A(X + D)} \notag\\
    &= \int d\Psi e^{i\Tr \Psi\Psi^{\dagger}J} \E_D e^{-i\Tr AD} \E_X e^{-i\Tr AX}.
\end{align}
$\E_D$ simply means integration against a delta-function density if $D$ is deterministic. 

\medskip
Let us introduce some notation: for $N\times N$ matrices $K$, $\Phi_X(K) = \E_X e^{-i\Tr XK}$, and similarly $\Phi_D$. We also define a new matrix ensemble $\bar{X} \overset{d}{=} O^T \Lambda O$, where $\Lambda=\text{diag}(\lambda_1, \ldots, \lambda_N)$ are equal in distribution to the eigenvalues of $X$ and $O$ is an entirely independent Haar-distributed orthogonal matrix.

Now
\begin{align}
   &\E_H Z_H(\j) = \int d\Psi e^{i\Tr \Psi\Psi^{\dagger}J} \Phi_{\bX}(K)\Phi_D(K) + \int d\Psi e^{i\Tr \Psi\Psi^{\dagger}J} (\Phi_X(K) - \Phi_{\bX}(K))\Phi_D(K)\notag\\
   \implies &\E G_{D+X}(z) = \E G_{D+\bX}(z) + \frac{1}{N}\frac{\partial}{\partial \j}\Bigg|_{\j = 0} \int d\Psi e^{i\Tr \Psi\Psi^{\dagger}J} (\Phi_X(K) - \Phi_{\bX}(K))\Phi_D(K) \equiv   \E G_{D+\bX}(z) + E(z)
\end{align}
and so we need to analyse the error term $E(z)$.\\

Now consider $X = U^T\Lambda U$ where the rows of $U$ are the eigenvectors $\{\vec{u}_i\}_i$ of $X$. Say also that $K = Q^TYQ$ for diagonal $Y = (y_1, \ldots, y_r, 0, \ldots, 0)$, where we note that $K$ has fixed rank, by construction. Then \begin{align*}
    \Tr XK = Y (UQ^T)^T\Lambda (UQ^T)
\end{align*}
but Lemma \ref{lem:que_preserved_under_rotation} establishes that the rows of $UQ^T$ obey QUE, since the rows of $U$ do. Further, Lemma \ref{lem:weaker_col_que} then establishes that the columns of $UQ^T$ obey $\hQUE$ as required by Lemma \ref{lem:explicit_error}. Let $\{\vec{v}_i\}$ be those columns, then we have \begin{align}\label{eq:trace_as_vsum}
    \Tr XK = \sum_{i=1}^r y_i \vec{v}_i^T \Lambda \vec{v}_i.
\end{align}


The expectation over $X$ can be split into eigenvalues and conditional eigenvectors 
\begin{align}\label{eq:phix_expansion}
    \Phi_X(K) = \E_{\Lambda}\E_{U\mid \Lambda}\sum_{l=0}^{\infty} \frac{1}{l!} (-i)^l\left(\Tr U^T \Lambda UK\right)^l.
\end{align}
We can simply bound \begin{align}
   \left| \sum_{l=0}^{n} \frac{1}{l!} (-i)^l\left(\Tr U^T \Lambda U\right)^l\right| \leq e^{|\Tr U^T\Lambda UK}
\end{align}
for any $n$, but clearly \begin{align}
    \E_{U\mid \Lambda}e^{|\Tr U^T\Lambda UK|} < \infty
\end{align}
since, whatever the distribution of $U\mid\Lambda$, the integral is over a compact group (the orthogonal group $O(N)$) and the integrand has no singularities. 
Therefore, by the dominated convergence theorem
\begin{align}
     \Phi_X(K) = \E_{\Lambda}\sum_{l=0}^{\infty} \frac{1}{l!} (-i)^l\E_{U\mid \Lambda}\left(\Tr U^T \Lambda UK\right)^l
\end{align}
and in precisely the same way
\begin{align}\label{eq:phibx_expansion}
      \Phi_X(K) = \E_{\Lambda}\sum_{l=0}^{\infty} \frac{1}{l!} (-i)^l\E_{O\sim \mu_{Haar}}\left(\Tr O^T \Lambda OK\right)^l.
\end{align}
Recalling (\ref{eq:trace_as_vsum}) we now have
\begin{align}\label{eq:phix_conditional_expansion}
    \Phi_X(K) = \E_{\Lambda}\sum_{l=0}^{\infty} \frac{1}{l!} (-i)^l \E_{U\mid \Lambda}\left(\sum_{i=1}^r y_i \vec{v}_i^T \Lambda \vec{v}_i\right)^l.
\end{align}
and similarly 
\begin{align}\label{eq:phixbar_conditional_expansion}
    \Phi_{\bX}(K) = \E_{\Lambda}\sum_{l=0}^{\infty} \frac{1}{l!} (-i)^l \E_{U\mid \Lambda}\left(\sum_{i=1}^r y_i \bar{\vec{v}}_i^T \Lambda \bar{\vec{v}}_i\right)^l.
\end{align}
where the $\bar{\vec{v}}_i$ are defined in the obvious way from $\bX$.
We would now apply $\hQUE$, but to do so we must insist that $\E_{\Lambda}$ is taken over the \emph{ordered} eigenvalues of $X$.
Having fixed that convention, lemma \ref{lem:explicit_error} can be applied to the terms 
\begin{align}
    \E_{U\mid \Lambda}\left(\sum_{i=1}^r y_i \vec{v}_i^T \Lambda \vec{v}_i\right)^l
\end{align}
in (\ref{eq:phix_conditional_expansion}).
The terms in $\Phi_{\bX}$ can be treated similarly.
This results in \begin{align}
    \Phi_X(K) - \Phi_{\bX}(K) &= \E_{\Lambda}\Bigg[\sum_{l=0}^{\infty} \frac{i^l}{l!} \left\{\E_{\{\vec{g}_i\}_{i=1}^r}\left(\sum_{i=1}^r y_i \frac{1}{N}\vec{g}_i^T\Lambda \vec{g}_i\right)^l + \left(\sum_{i=1}^r N^{-(1+\epsilon)} y_i \vec{\eta}_i^T\Lambda \vec{\eta}_i\right)^l \right\}\notag\\
    & ~~~~~~~~-\sum_{l=0}^{\infty} \frac{i^l}{l!} \left\{\E_{\{\vec{g}_i\}_{i=1}^r}\left(\sum_{i=1}^r y_i \frac{1}{N}\vec{g}_i^T\Lambda \vec{g}_i\right)^l + \left(\sum_{i=1}^r N^{-(1+\epsilon)} y_i \bar{\vec{\eta}}_i^T\Lambda \bar{\vec{\eta}}_i\right)^l \right\}\Bigg]
\end{align}
The exponential has infinite radius of convergence, so we may re-order the terms in the sums to give cancellation
\begin{align*}
    \Phi_X(K) - \Phi_{\bX}(K) = \E_{\Lambda}\sum_{l=1}^{\infty}\frac{1}{l!} N^{-(1+\epsilon)l}(-i)^l\left(\sum_{i=1}^r y_i \vec{\eta}_i^T\Lambda \vec{\eta}_i\right)^l -\E_{\Lambda}\sum_{l=1}^{\infty}\frac{1}{l!} N^{-(1+\epsilon)l}(-i)^l\left(\sum_{i=1}^r y_i \bar{\vec{\eta}}_i^T\Lambda \bar{\vec{\eta}}_i\right)^l.
\end{align*}
Here $\epsilon>0$ and $\vec{\eta}_i, \tilde{\vec{\eta}}_i\in \C^N$ with 
\begin{align}
   -1\leq [(\vec{\eta}_i)_j]^2 , [(\bar{\vec{\eta}}_i)_j]^2 \leq 1 ~&~ \forall i=1,\ldots, r, ~  \forall j\in\TN,\\
   -N^{\epsilon}\leq [(\vec{\eta}_i)_j]^2 , [(\bar{\vec{\eta}}_i)_j]^2 \leq N^{\epsilon} ~&~ \forall i=1,\ldots, r, ~  \forall j\in\TN.
\end{align}

Simplifying, we obtain \begin{align}
    \Phi_X(K) - \Phi_{\bX}(K) = \E_{\Lambda}\exp\left(-iN^{-(1+\epsilon)}\sum_{i=1}^r y_i \vec{\eta}_i^T\Lambda \vec{\eta}_i\right) - \E_{\Lambda}\exp\left(-iN^{-(1+\epsilon)}\sum_{i=1}^r y_i \tilde{\vec{\eta}}_i^T\Lambda \tilde{\vec{\eta}}_i\right).
\end{align}
Since $|\TN^c| \leq 2N^{1-\delta}$ we have \begin{align}
    \sum_{j\in\TN^c} |\lambda_j| \leq \mathcal{O}(N^{1-d} N^{-1}) \Tr |\Lambda|
\end{align}
and so \begin{align}
    |\vec{\eta}_i^T\Lambda \vec{\eta}_i| \leq \Tr|\Lambda|\left( 1 + \mathcal{O}(N^{\epsilon - \delta})\right).
\end{align}
For any fixed $\delta>0$, $\epsilon$ can be reduced if necessary so that $\epsilon < \delta$ and then for sufficiently large $N$ we obtain, say, 
\begin{align}
    |\vec{\eta}_i^T\Lambda \vec{\eta}_i| \leq 2 \Tr|\Lambda|.
\end{align}
Thence we can write $\vec{\eta}_i^T\Lambda\vec{\eta}_i = \Tr|\Lambda| \xi_i$ for $\xi_i\in[-2, 2]$, and similarly $\tilde{\vec{\eta}}_i^T\Lambda\tilde{\vec{\eta}}_i = \Tr|\Lambda| \tilde{\xi}_i$. Now
\begin{align*}
    \E_{\Lambda}\exp\left(-iN^{-(1+\epsilon)} \sum_{i=1}^r \xi_iy_i\int \Tr|\Lambda|\right)=\E_{\Lambda}\exp\left(-iN^{-\epsilon} \sum_{i=1}^r \xi_iy_i\int d\hat{\mu}_X(\lambda)|\lambda|\right)
\end{align*}
so we can apply Laplace's method to the empirical spectral measure $\hat{\mu}_X$ to obtain \begin{align}
    \E_{\Lambda}\exp\left(-iN^{-(1+\epsilon)} \sum_{i=1}^r \xi_iy_i\int \Tr|\Lambda|\right)=\exp\left(-iN^{-\epsilon} (q+o(1))\sum_{i=1}^r \xi_iy_i\right) + o(1)
\end{align}
where the $o(1)$ terms do not depend on the $y_i$ and where we have defined \begin{align}
    q = \int d\mu_X(\lambda)|\lambda|.
\end{align}
Further, we can write $\sum_{i=1}^r \xi_i y_i = \zeta\Tr K$, where $\zeta \in [\min_i\{\xi_i\}, \max_i\{\xi_i\}]\subset [-1, 1]$, and similarly $\sum_{i=1}^r \tilde{\xi}_i y_i = \tilde{\zeta}\Tr K$. Then \begin{align}
    \Phi_X(K) - \Phi_{\bX}(K) = e^{-iN^{-\epsilon}\zeta (q + o(1)) \Tr K} - e^{-iN^{-\epsilon}\tilde{\zeta} (q + o(1)) \Tr K} + o(1)
\end{align}
but
\begin{align}
    \frac{1}{N}\frac{\partial}{\partial \j}\Bigg|_{\j=0}\int d\Psi e^{i\Tr \Psi\Psi^{\dagger}J}e^{-iN^{-\epsilon}\zeta (q + o(1)) \Tr K}\Phi_D(K) &= \E G_{D + N^{-\epsilon}\zeta(q + o(1))I}(z)
\end{align}
and so $E(z) = o(1)$. We have thus established that \begin{align}
    \E G_{D+X}(z) = \E G_{D+\bX}(z) + o(1)
\end{align}
from which one deduces that $\mu_{D+X} = \mu_{D + \bX} = \mu_D \boxplus \mu_{\bX} = \mu_D\boxplus\mu_X$.
\end{proof}

\begin{rem}
We have also constructed a non-rigorous argument for Theorem \ref{thm:nearly_free_addn} where the supersymmetric approach is replaced by the replica method. This approach simplifies some of the analysis and allows one to prove agreement between the resolvents themselves, not just the traces.
\end{rem}
% Now define a random matrix $Y\overset{d}{=}U^T\Lambda U$ where $U$ is a Haar distributed orthogonal matrix and $\Lambda$ is equal in distribution to the diagonal matrix of eigenvalues of $X$. By construction $\mu_X = \mu_Y$. From (\ref{eq:phi_k_haar_equivalent}), using the local law on $X$, we have the result from Appendix section \ref{sec:fourier}
% \begin{align}
%     |\E_X e^{-i\Tr AX} - \E_Y  e^{-i\Tr AY}| \lesssim N^{-\epsilon(\{a_i\})}
% \end{align}
% and so we have to somehow carve up the domain of integration of $\Psi$ so that 
% \begin{align}
%     \int d\Psi e^{i\Tr \Psi\Psi^{\dagger}J} e^{-i\Tr AD} N^{-\epsilon(\{a_i\})} = N^{-\epsilon'} + \text{exp. small. term}
% \end{align}
% for some $\epsilon'>0$, which would then suffice to show \begin{align}
%     \left|\frac{1}{N}\langle G_X(z)\rangle - \frac{1}{N}\langle G_Y(z)\rangle \right| \lesssim N^{-\epsilon'}.
% \end{align}
% This result is sufficient to show that the limiting spectral measure of $X+D$ is the same as $Y+D$ which is known to be $\mu_{X}\boxplus \mu_D$. Moreover, it shows that a local law for $Y+D$ transfers to $X+D$.

\subsection{Experimental validation} ~\\

We consider the following matrix ensembles:
\begin{align*}
    M\sim GOE^n ~ &: ~ \text{Var}(M_{ij}) = \frac{1 + \delta_{ij}}{2n},\\
    M\sim UWig^n &: ~ \sqrtsign{n}M_{ij} \overset{i.i.d}{\sim} U(0, \sqrtsign{6}) ~~\text{up to symmetry},\\
    M\sim \Gamma Wig^n &: ~ 2\sqrtsign{n}M_{ij} \overset{i.i.d}{\sim} \Gamma(2) ~~\text{up to symmetry},\\
    M\sim UWish^n &: ~ M\overset{d}{=}\frac{1}{m}XX^T, ~ X_{ij}\overset{i.i.d}{\sim}U(0, \sqrtsign{12}) ~~\text{for }X\text{ of size }n\times m, ~~ \frac{n}{m} \overset{n,m\rightarrow\infty}{\rightarrow} \alpha.
\end{align*}

All of the $GOE^n, UWig^n, \Gamma Wig^n$ have the same limiting spectral measure, namely $\mu_{SC}$, the semi-circle of radius $\sqrtsign{2}$. $UWish^n$ has a Marcenko-Pastur limiting spectral measure $\mu_{MP}$, and the constant $\sqrtsign{12}$ is chosen so that the parameters of the MP measure match those of a Gaussian Wishart matrix for which $X$ has the same aspect ratio and has standard Gaussian entries. $GOE^n$ is the only ensemble whose eigenvectors are Haar distributed, but all ensembles obey a local law in the sense above. It is known that the sum of $GOE^n$ and any of the other ensembles will have limiting spectral measure given by the free additive convolution of $\mu_{SC}$ and the other ensemble's measure (so either $\mu_{SC}\boxplus\mu_{MP}$ or $\mu_{SC}\boxplus\mu_{SC}$). Our result implies that the same holds for addition of the non-invariant ensembles. Sampling from the above ensembles is simple, so we can easily generate spectral histograms from multiple independent matrix samples for large $n$. $\mu_{SC}\boxplus\mu_{SC}$ is just another semi-circle measure but with radius $2$. $\mu_{SC}\boxplus\mu_{MP}$ can be computed in the usual manner with $R$-transforms and is given by the solution to the polynomial \begin{align*}
    \frac{\alpha}{2}t^3 - \left(\frac{1}{2} + \alpha z\right)t^2 + (z + \alpha - 1)t - 1 = 0.
\end{align*}
i.e. Say the cubic has roots $\{r_1, r_2 + is_2, r_2 - is_2\}$ for $s_2\geq 0$, then the density of $\mu_{SC}\boxplus\mu_{MP}$ at $z$ is $s_2/\pi$. This can all be solved numerically. The resulting plots are in Figure \ref{fig:free_sum_comparison} and clearly show agreement between the free convolutions and sampled spectral histograms.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.3\linewidth}
        \includegraphics[width=\textwidth]{wigner_wishart_que.pdf}
        \subcaption{ $UWig^n + UWish^n$}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
        \includegraphics[width=\textwidth]{wigner_wishart_gamma_unif_que.pdf}
        \subcaption{ $\Gamma Wig^n + UWish^n$}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
        \includegraphics[width=\textwidth]{wigner_wigner_que.pdf}
        \subcaption{ $UWig^n + \Gamma Wig^n$}
    \end{subfigure}
    \caption{Comparison of theoretical spectral density and empirical from sampled matrices all of size $500\times 500$. We combine $50$ independent matrix samples per plot.}
    \label{fig:free_sum_comparison}
\end{figure}

We can also test the result in another more complicated case. Consider the case of random $d$-regular graphs on $N$ vertices. Say $M\sim Reg^{N,d}$ is the distribution of the adjacency matrix of such random graphs. The limiting spectral density of $M\sim Reg^{N,d}$ is known in closed form, as is its Stieljtes transform \cite{bauerschmidt2019local}. Moreover, \cite{bauerschmidt2019local} established a local law of the kind required for our results. Let $\mu_{KM}^{(d)}$ be the Kesten-McKay law, the limiting spectral measure of $d$-regular graphs. We can find an explicit degree-6 polynomial for the Stieljtes transform of $\mu_{KM}^{(d)}\boxplus \mu_{SC}$ which is then amenable to straightforward numerical solution. Moreover, there are known efficient algorithms for sampling random $d$-regular graphs \cite{kim2003generating, steger1999generating} along with implementations \cite{SciPyProceedings_11}.

\medskip
Alternatively we can investigate agreement with $\mu_{KM}^{(d)}\boxplus \mu_{SC}$ indirectly by sampling spectra from say $Reg^{N,d} + UWig^N$ and also from  $Reg^{N,d} + GOE^N$.
The latter case will certainly yield the distribution $\mu_{KM}^{(d)}\boxplus \mu_{SC}$ since the GOE matrices are freely independent from the adjacency matrices.
Figure shows a q-q plot for samples from these two matrix distributions and demonstrates near-perfect agreement, thus showing that indeed the spectrum of $Reg^{N,d} + UWig^N$  is indeed described by $\mu_{KM}^{(d)}\boxplus \mu_{SC}$.

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{haar-vs-que-regular_graph.pdf}
    \caption{q-q plot comparing the spectrum of samples from $Reg^{N,d} + UWig^N$ ($y$-axis) to samples from $Reg^{N,d} + GOE^N$ ($x$-axis).}
    \label{fig:qq_plot}
\end{figure}

==> application.tex <==
%auto-ignore
\section{Application to machine learning}
\subsection{Global complexity} ~\\

Consider a loss function $L(\vec{w}; \vec{x}, y)$ for weights $\vec{w}\in\mathbb{R}^N$, input data point $\vec{x}\in\mathbb{R}^D$ and target value $y\in \mathbb{R}^c$. Now introduce a random function $\L$ due to the random sampling of the data in a batch, i.e. 
\begin{align}
    \L(\vec{w}) \overset{d}{=} \frac{1}{n_b} \sum_{i=1}^{n_b} L(\vec{w}; \vec{x}_i, y_i), ~~ (\vec{x}_i, y_i)\overset{i.i.d}{\sim} \mathbb{P}_{\text{data}}.
\end{align}

$\L$ is the training loss with batch size $n_b$. We can always write \begin{align}
    \L(\vec{w}) = \bL(\vec{w}) + \hL(\vec{w})
\end{align}
where we define $\bL = \E L$ and $\hL = \L - \bL$, the expectation being taken with respect to the data distribution. Here $\bL$ is the true loss and $\hL$ is the batch-wise random noise in the loss. Now define the Hessians \begin{align}
    D(\vec{w}) = \nabla^2 \bL(\vec{w}), ~~ X(\vec{w}) = \nabla^2 \hL(\vec{w})\mid \{\nabla \L = 0\}.
\end{align}
Here $D$ is a deterministic $N\times N$ matrix function of $\vec{w}$ and $X$ is a random $N\times N$ matrix function of $\vec{w}$. Now define the complexity for sets $\B\subset \R^N$ \begin{align}
    C_N(\B) = |\{ \vec{w}\in \B \mid \nabla \L(\vec{w}) = 0\}|.
\end{align}
This is simply the number of stationary points of the training loss in the region $\B$ of weight space. Under appropriate conditions on $X$ (which one could determine from \cite{adler2007random}, or just be non-rigorous and gloss over) we have
\begin{align}\label{eq:w_b_dom_integral_kacrice}
    \E C_N = \int_{\B} d\vec{w} ~ \phi_{\vec{w}}(-\nabla \bL) \E |\det (D + X)|
\end{align}
where $\phi_{\vec{w}}$ is the density of $\nabla\hL$ at $\vec{w}$. Again, we get the conditions from \cite{arous2021exponential} or just gloss over and say that generically \begin{align*}
    \frac{1}{N}\log\E |\det (D + X)| \sim \int d\mu_{X+D}(\lambda) \log |\lambda|.
\end{align*}
By our other results, a local law on $X$ is sufficient to give $\mu_{X+D} = \mu_X \boxplus \mu_D$. We want to apply the Laplace method to the integral in (\ref{eq:w_b_dom_integral_kacrice}). We need to deal with the gradient density $\phi_{\vec{w}}(-\nabla\bL)$ somehow. For instance, we could assume that $\B$ contains a single zero $\vec{w}^*$ of the true loss gradient $\bL$. We could also assume that the gradient noise density $\phi_{\vec{w}}$ is has a single mode at $0$. We may then perhaps reduce $\phi_{\vec{w}}(-\nabla\bL(\vec{w}))$ to a function of fixed dimensional function of $\vec{w}$, e.g. $\|\vec{w} - \vec{w}^*\|_2$. Applying the Laplace method combined with Kac-Rice then generically says that $\E C_N(\B)$ is either exponentially large like $e^{+cN}$ or exponentially small like $e^{-cN}$.

\medskip
Experimental results suggest that the spectrum $\mu_{X+D}$ starts broad and becomes quite strongly peaked around $0$ as training progresses. We may therefore expect that $\int d\mu_{X+D}(\lambda)\log|\lambda|$ moves from positive to negative as training progresses (note that the integral is a function of $\vec{w}$, since the measure is). The more negative this integral is, the more it encourages $\E C_N(\B)$ to be exponentially small. 

\medskip
The overall picture is then of a training loss surface consisting of a patchwork of regions or two types: smooth (i.e. essentially no critical points due to the noise term) and rough (i.e. exponentially many critical points due to the noise term). Moreover, empirical observations about the Hessian imply that we expect that training moves $\vec{w}$ to smooth regions.

\medskip Given this picture, a natural question is what do the boundaries between these regions look like? I.e. what regime interpolates between $e^{+cN}$ many critical points and $e^{-cN}$ few critical points? The boundaries correspond to \begin{align*}
     \int d\mu_{X+D}(\lambda) \log |\lambda| = 0.
\end{align*}
The question is then is to consider \begin{align*}
    \frac{1}{N}\log \E|\det H| - \int d\mu_H(\lambda)\log|\lambda|
\end{align*}
for general random matrix ensembles $H$, e.g. with a local law. Can we at least get its order of magnitude?
% To make a little progress we will assume $\hL$ is a Gaussian process. $C_N$ is computed using the Kac-Rice formula (the Gaussianity of $\hL$ guarantees we can apply this result)
% \begin{align}
%     \E C_N = \int_{\B} d\vec{w} ~ \phi_{\vec{w}}(0) \E |\det (D + X)|
% \end{align}
% where $\phi_{\vec{w}}$ is the density of $\nabla \L(\vec{w})$. The Gaussianity of $\nabla \L$ will help to keep $\E C_N$ finite. Let us say $\phi_{\vec{w}}(\vec{x}) \propto \exp\left\{-\frac{N}{2}(\vec{v}(\vec{w}) - \vec{x})^T\Sigma(\vec{w})^{-1}(\vec{v}(\vec{w}) - \vec{x})\right\}$

% \medskip
% We need to make assumptions on $X$ in order to apply the theorems of \cite{arous2021exponential}. In particular we assume the existence of $\mu_X$, the limiting spectral measure of $X$. Note this will be parametrised by $\vec{w}$ in general. We also assume that $\mu_X$ has compact support for all $\vec{w}$ and that it obeys a local law. These are all reasonable assumptions for a noise model, and in particular the local law ensures that the eigenvalues spacings of $X$ have universal GOE statistics. Let $\mu_D$ be the limiting spectral measure of $D$. Our result in the previous section then combines with Theorem 4.1 of \cite{arous2021exponential} to give 
% \begin{align}
%     \lim_{N\rightarrow \infty}\frac{1}{N}\log \E C_N(\B) = \sup_{\vec{w}\in\B}\left\{ -\frac{1}{2}\vec{v}(\vec{w})^T\Sigma(\vec{w})^{-1}\vec{v}(\vec{w}) + \int \mu_{X+D}(\vec{w})(d\lambda)\log|\lambda|\right\}
% \end{align}
% where we have $\mu_{X+D}=\mu_X\boxplus\mu_D$. Note that $\vec{v}(\vec{w}) = \nabla \bL(\vec{w})$. Now suppose that $D(\vec{w})$ is low rank for all $\vec{w}$, i.e. $\text{rank}(D(\vec{w})) = o(N)$ for all $\vec{w}$. The $\mu_D = \delta$ and so $\mu_{X+D} = \mu_X$. Overall
% \begin{align}
%     \lim_{N\rightarrow \infty}\frac{1}{N}\log \E C_N(\B) = \sup_{\vec{w}\in\B}\left\{ -\frac{1}{2}\nabla\bL(\vec{w})^T\Sigma(\vec{w})^{-1}\nabla\bL(\vec{w}) + \int \mu_{X}(\vec{w})(d\lambda)\log|\lambda|\right\}.
% \end{align}

\subsection{Outliers} ~\\

Let $\{\lambda_i\}$ be the eigenvalue of $X+D$ and say $D$ has ordered eigenvalues $(\tau_1, \ldots, \tau_r, 0, \ldots, 0, \nu_s, \ldots, \nu_1)$. If $X$ had Haar eigenvectors, then the results of \cite{benaych2011eigenvalues} would give \begin{align}
    \lambda_j \overset{a.s.}{\rightarrow} \begin{cases}
                    G_{\mu_X}^{-1}(\nu_j^{-1}) ~~&\text{if } \nu_j > 1/G_{\mu_X}(\mathtt{r}(\mu_X)),\\
                    \mathtt{r}(\mu_X) &\text{otherwise},
                \end{cases}\label{eq:outlier_1}\\
    \lambda_{N-j+1} \overset{a.s.}{\rightarrow} \begin{cases}
                    G_{\mu_X}^{-1}(\tau_j^{-1}) ~~&\text{if } \tau_j < 1/G_{\mu_X}(\mathtt{l}(\mu_X)),\\
                    \mathtt{l}(\mu_X) &\text{otherwise},
                \end{cases}\label{eq:outlier_2}                
\end{align}
where $\mathtt{r}(\mu_X), \mathtt{l}(\mu_X)$ are the left and right edges of the support of $\mu_X$ respectively. It was conjectured in \cite{benaych2011eigenvalues} that (\ref{eq:outlier_1}) and (\ref{eq:outlier_2}) still hold when $X$ has delocalised eigenvectors, rather than strictly Haar. There are some results available CITATIONS, but for completeness, we prove the generalisation in Appendix \ref{sec:outlier_gen}.

\medskip
Now recall that $\hL$ is the error in the loss due to taking a random finite batch of data points. Let us replace therefore $X$ with $g(n_b)X$, where $X$ is now the error term for a batch size of $1$, and $g$ is some function $\N \rightarrow (0, \infty)$ which measure the effect of batch size on the variance of the error term. It is simple to show $G_{g(n_b)\mu_X}(z) = G_{\mu_X}(z/g(n_b))$, from which it follows 
\begin{align}
    \lambda_j \overset{a.s.}{\rightarrow} g(n_b)\begin{cases}
                    G_{\mu_X}^{-1}(\nu_j^{-1}) ~~&\text{if } \nu_j > 1/G_{\mu_X}(\mathtt{r}(\mu_X)),\\
                    \mathtt{r}(\mu_X) &\text{otherwise},
                \end{cases}\label{eq:outlier_batch_1}\\
    \lambda_{N-j+1} \overset{a.s.}{\rightarrow} g(n_b)\begin{cases}
                    G_{\mu_X}^{-1}(\tau_j^{-1}) ~~&\text{if } \tau_j < 1/G_{\mu_X}(\mathtt{l}(\mu_X)),\\
                    \mathtt{l}(\mu_X) &\text{otherwise}.
                \end{cases}\label{eq:outlier_batch_2}                
\end{align}
There are several important features of (\ref{eq:outlier_batch_1}) and (\ref{eq:outlier_batch_2}):
\begin{enumerate}
    \item The scaling $g(n_b)$ can be examined directly from real data by simply looking at the size of the top eigenvalues of neural network Hessians for various batches sizes. It is known that the spectrum broadens as batch size decreases.
    \item The scaling is shared between all the outliers. 
    \item The conditions on $\nu_j, \tau_j$ for the outliers to exist are independent of the batch size. 
\end{enumerate}

Our model makes three assumption: $D$ is low-rank, $X$ obeys a local law, and the simple multiplicative effect of the batch size through $g(n_b)$. Testing the first of these assumptions would require, in principle, infinitely-many samples from distribution of the batch Hessian, though \cite{granziol2020learning} provide some indicative results in this direction, showing that $D$ does indeed to be approximately low-rank for real deep neural networks. The local law assumption is yet more difficult to assess. If the dimension of the Hessian were not too large, one could compute exact eigen-decompositions of samples from its distribution and, for example, investigate local spectral statistics as done in \cite{baskerville2022appearance}. However, for deep neural networks of the greatest practical interest, the Hessian would be much too large even to compute the Hessian, let alone its eigen-decomposition.

\medskip
Point 2 above, however, suggests an indirect means of testing our assumptions on large deep neural networks. Indeed, we can use Lanczos power methods to compute good approximations to the top few outliers in the batch Hessian spectra of deep neural networks \cite{granziol2020learning}. Over a range of batch sizes, we compute the top 5 outliers of the batch Hessian for 10 different batch seeds. We repeat this procedure at various epochs throughout the training of a VGG16 image classifier on the CIFAR100 dataset, in particular epoch 0 (initialisation), epoch 50, epoch 150 and epoch 300 (final epoch). By the end of training at epoch 300, the model has a test of accuracy of INSERT ACCURACY. Let $\lambda^{(i, j, e)}_n$ be the top $i$-th outlier (so $i=1$ is the top outlier) for the $j$ batch seed and a batch size of $n$ for the model at epoch $e$. 

\medskip
Rather than analysing the agreement of the data $\lambda^{(i, j, e)}_n$ with (\ref{eq:outlier_batch_1}), we first develop a generalisation of the model in which the low-rank assumption for $D$ is loosened.
A full generalisation to this case is not possible without entirely losing the the outlier structure in (\ref{eq:outlier_batch_1}), so we must consider the case where $D$ has fixed rank in some approximate sense.
Indeed, let us suppose that $D$ has outlier eigenvalues $0<\nu_s< \ldots, \nu_1$ and remaining eigenvalues $\xi_1,\ldots, \xi_{N-s}$. Further, let us suppose that \begin{align}
    \frac{1}{N}\sum_{j=1}^{N-s}\delta_{\xi_j} \rightarrow \mu_E \text{ as } N\rightarrow\infty
\end{align}
for some measure $\mu_E$. Note that $\mu_E$ is deterministic because $D$ is. To make precise the notion of approximate fixed rank for $D$, we assume \begin{align}
    \mu_E = \epsilon\omega + (1-\epsilon)\delta_0
\end{align}
where $\epsilon>0$ is small and $\omega$ is supported on $(-\eta, \eta)$ for some $\eta>0$. As $\epsilon\rightarrow 0$ $\mu_E$ approaches $\delta_0$, corresponding to $\text{rank}(D) = o(N)$. Write $H = O^TLO$ where $L = \text{diag}(\nu_1, \ldots, \nu_s, \xi_1, \ldots, \xi_{N-s})$ and $O$ is an orthogonal matrix. $H$ has the same spectrum as $Z = L + OXO^T$, and $OXO^T$ obeys a local law with measure $\mu_X$ \draft{justify}. By Theorem \ref{thm:nearly_free_addn} $Z$ has limiting spectral measure $\mu_X \boxplus \mu_E$ and \draft{justify} obeys a local law. We have \begin{align}
    B_Z(z) = \frac{1}{z} + R_{g(n_b)X}(z) + R_{\mu_E}(z) = g(n_b) B_{\mu_X}(z) - \frac{1}{z} + B_{\mu_E}(z)
\end{align}
and 
\begin{align}
    G_{\mu_E}(z) = \frac{1-\epsilon}{z} + \epsilon G_{\omega}(z).
\end{align}
We seek a solution of the form \begin{align}
    B_{\mu_E}(z) = \frac{1}{z} + \epsilon f(z) 
\end{align}
which requires \begin{align}
    z &= (1-\epsilon)\left(z^{-1} + \epsilon f(z)\right)^{-1} + \epsilon G_{\omega}\left(z^{-1} + \epsilon f(z)\right)\notag\\
    &= z - \epsilon\left[z + f(z) - G_{\omega}(z^{-1})\right] + \mathcal{O}(\epsilon^2)
\end{align}
so $f(z) = G_{\omega}(z^{-1}) - z + \mathcal{O}(\epsilon)$, but \begin{align}
    G_{\omega}(z) = \int \frac{d\omega(\lambda)}{z- \lambda}
\end{align}
and so our solution for $B_{\mu_E}(z)$ is valid so long as $d(z^{-1}, [-\eta, \eta]) > 0$, i.e. the Euclidean distance in $\mathbb{C}$ between $z^{-1}$ and its closest point in $[-\eta, \eta]$, the support of $\omega$.
The RAO-THEOREM result now gives the following result for the outliers of $H$:

\begin{align}
    \lambda_j \overset{a.s.}{\rightarrow} \begin{cases}
                     g(n_b)G_{\mu_X}^{-1}(\nu_j^{-1}) + \epsilon(G_{\omega}(\nu_j) - \nu_j^{-1}) + \mathcal{O}(\epsilon^2) ~~&\text{if } \nu_j > 1/G_{\mu_Z}(\mathtt{r}(\mu_Z)),\\
                    \mathtt{r}(\mu_Z) &\text{otherwise},
                \end{cases}\label{eq:outlier_perturbed_batch_1}
    % \lambda_{N-j+1} \overset{a.s.}{\rightarrow} g(n_b)\begin{cases}
    %                 G_{\mu_X}^{-1}(\tau_j^{-1}) ~~&\text{if } \tau_j < 1/G_{\mu_X}(\mathtt{l}(\mu_X)),\\
    %                 \mathtt{l}(\mu_X) &\text{otherwise}.
    %             \end{cases}\label{eq:outlier_batch_2}                
\end{align}
provided that $ \nu_j> \eta$. To determine the the support of $\mu_Z$, let us seek a solution of the form $\mathtt{r}(\mu_Z) = g(n_b)\mathtt{r}(\mu_X) + \delta$. Then (\ref{eq:outlier_perturbed_batch_1}) provides a consistency condition at $\nu_j = 1/G_{\mu_Z}(\mathtt{r}(\mu_Z))$  which implies $\delta = \mathcal{O}(\epsilon)$.
The key observation from the result (\ref{eq:outlier_perturbed_batch_1}) is that the outliers of $H$ no longer have a simple scaling behaviour by $g(n_b)$ with batch size, but a shifted version thereof. 

\medskip 
To compare the experimental results to our theoretical model, we propose a shifted power law $l^{(i,e)}n^{-\frac{1}{2}} + d^{(i,e)}$. The power $-\frac{1}{2}$ is the value that one would get in the case of Gaussian $X$ and was the value used in \cite{granziol2020learning}, but is used here for convenience and because attempts to numerically fit such values to the data could result in spurious values not adequately supported by the data. The constants $l^{(i,e)}$ correspond to $G_{\mu_X}^{-1}(\nu_i^{-1})$ where both $\nu_i$ and $\mu_X$ can vary with epoch, and $d^{(i,e)}$ corresponds to $\epsilon(G_{\omega}(\nu_i) - \nu_i^{-1})$ where $\epsilon$ and $G_{\omega}$ can also vary with epoch. The constants $l^{(i,e)}, d^{(i,e)}$ could be selected by minimising mean squared error, for example, but we instead select them as solutions to the linear system \begin{align}
    \frac{1}{10}\sum_{j=1}^{10}  \lambda^{(i, j, e)}_{n_1} &= l^{(i, e)}n_1^{-\frac{1}{2}} + d^{(i, e)},\\
   \frac{1}{10} \sum_{j=1}^{10} \lambda^{(i, j, e)}_{n_2} &= l^{(i, e)}n_2^{-\frac{1}{2}} + d^{(i, e)},
\end{align}
where $n_1=1024$ and $n_2=512$ are the two largest batch sizes considered. This method was chosen as the largest batch sizes have the smallest variance between batch seeds, making the sample means good estimates. 

The results are show in Figure \ref{fig:outlier_fit}. We see excellent agreement between the model and the data for epoch 0. For epochs 50 (early in training) and epoch 150 (halfway through training) the agreement is noticeably degraded at small batch sizes, however this appears to be due to increased variance between batch seeds. At epoch 300 (final trained model), the agreement is very poor beyond the first outlier.
\begin{figure}[h]
    \centering
    \begin{subfigure}{0.25\linewidth}
     \centering
     \includegraphics[width=\linewidth]{simple_epoch=0_outlier=1_fit_single.pdf}
     \subcaption{Outlier 1, epoch 0}
    \end{subfigure}
    \begin{subfigure}{0.25\linewidth}
     \centering
     \includegraphics[width=\linewidth]{simple_epoch=0_outlier=2_fit_single.pdf}
     \subcaption{Outlier 2, epoch 0}
    \end{subfigure}
    \begin{subfigure}{0.25\linewidth}
     \centering
     \includegraphics[width=\linewidth]{simple_epoch=0_outlier=5_fit_single.pdf}
     \subcaption{Outlier 5, epoch 0}
    \end{subfigure}
    
    \begin{subfigure}{0.25\linewidth}
     \centering
     \includegraphics[width=\linewidth]{simple_epoch=50_outlier=1_fit_single.pdf}
     \subcaption{Outlier 1, epoch 50}
    \end{subfigure}
    \begin{subfigure}{0.25\linewidth}
     \centering
     \includegraphics[width=\linewidth]{simple_epoch=50_outlier=2_fit_single.pdf}
     \subcaption{Outlier 2, epoch 50}
    \end{subfigure}
    \begin{subfigure}{0.25\linewidth}
     \centering
     \includegraphics[width=\linewidth]{simple_epoch=50_outlier=5_fit_single.pdf}
     \subcaption{Outlier 5, epoch 50}
    \end{subfigure}
    
    \begin{subfigure}{0.25\linewidth}
     \centering
     \includegraphics[width=\linewidth]{simple_epoch=150_outlier=1_fit_single.pdf}
     \subcaption{Outlier 1, epoch 150}
    \end{subfigure}
    \begin{subfigure}{0.25\linewidth}
     \centering
     \includegraphics[width=\linewidth]{simple_epoch=150_outlier=2_fit_single.pdf}
     \subcaption{Outlier 2, epoch 150}
    \end{subfigure}
    \begin{subfigure}{0.25\linewidth}
     \centering
     \includegraphics[width=\linewidth]{simple_epoch=150_outlier=5_fit_single.pdf}
     \subcaption{Outlier 5, epoch 150}
    \end{subfigure}
    
    \begin{subfigure}{0.25\linewidth}
     \centering
     \includegraphics[width=\linewidth]{simple_epoch=300_outlier=1_fit_single.pdf}
     \subcaption{Outlier 1, epoch 300}
    \end{subfigure}
    \begin{subfigure}{0.25\linewidth}
     \centering
     \includegraphics[width=\linewidth]{simple_epoch=300_outlier=2_fit_single.pdf}
     \subcaption{Outlier 2, epoch 300}
    \end{subfigure}
    \begin{subfigure}{0.25\linewidth}
     \centering
     \includegraphics[width=\linewidth]{simple_epoch=300_outlier=5_fit_single.pdf}
     \subcaption{Outlier 5, epoch 300}
    \end{subfigure}
    \centering
    \caption{The batch-size scaling of the outliers in the spectra of the Hessians of the VGG16 loss on CIFAR10. Training epochs increase top-to-bottom from initialisation to final trained model. Left-to-right the outlier index varies (outlier 1 being the largest). Red cross show results from Lanczos approximations over 10 samples (different batches) for each batch size. The blue lines are parametric power law fits of the form $y=\ell B^{-\kappa}$ where the parameter $\kappa$ is shared within each row, but a different parameter $\ell$ is used for each plot.}
    \label{fig:outlier_fit}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{0.25\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{epoch=0_outlier=1_fit_single_fixed.pdf}
%      \subcaption{Outlier 1, epoch 0}
%     \end{subfigure}
%     \begin{subfigure}{0.25\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{epoch=0_outlier=2_fit_single_fixed.pdf}
%      \subcaption{Outlier 2, epoch 0}
%     \end{subfigure}
%     \begin{subfigure}{0.25\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{epoch=0_outlier=5_fit_single_fixed.pdf}
%      \subcaption{Outlier 5, epoch 0}
%     \end{subfigure}
    
%     \begin{subfigure}{0.25\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{epoch=25_outlier=1_fit_single_fixed.pdf}
%      \subcaption{Outlier 1, epoch 25}
%     \end{subfigure}
%     \begin{subfigure}{0.25\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{epoch=25_outlier=2_fit_single_fixed.pdf}
%      \subcaption{Outlier 2, epoch 25}
%     \end{subfigure}
%     \begin{subfigure}{0.25\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{epoch=25_outlier=5_fit_single_fixed.pdf}
%      \subcaption{Outlier 5, epoch 25}
%     \end{subfigure}
    
%     \begin{subfigure}{0.25\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{epoch=150_outlier=1_fit_single_fixed.pdf}
%      \subcaption{Outlier 1, epoch 150}
%     \end{subfigure}
%     \begin{subfigure}{0.25\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{epoch=150_outlier=2_fit_single_fixed.pdf}
%      \subcaption{Outlier 2, epoch 150}
%     \end{subfigure}
%     \begin{subfigure}{0.25\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{epoch=150_outlier=5_fit_single_fixed.pdf}
%      \subcaption{Outlier 5, epoch 150}
%     \end{subfigure}
    
%     \begin{subfigure}{0.25\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{epoch=300_outlier=1_fit_single_fixed.pdf}
%      \subcaption{Outlier 1, epoch 300}
%     \end{subfigure}
%     \begin{subfigure}{0.25\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{epoch=300_outlier=2_fit_single_fixed.pdf}
%      \subcaption{Outlier 2, epoch 300}
%     \end{subfigure}
%     \begin{subfigure}{0.25\linewidth}
%      \centering
%      \includegraphics[width=\linewidth]{epoch=300_outlier=5_fit_single_fixed.pdf}
%      \subcaption{Outlier 5, epoch 300}
%     \end{subfigure}
%     \centering
%     \caption{The batch-size scaling of the outliers in the spectra of the Hessians of the VGG16 loss on CIFAR10. Training epochs increase top-to-bottom from initialisation to final trained model. Left-to-right the outlier index varies (outlier 1 being the largest). Red cross show results from Lanczos approximations over 10 samples (different batches) for each batch size. The blue lines are parametric power law fits of the form $y=\ell B^{-0.5}$ where different parameter $\ell$ is used for each plot.}
%     \label{fig:outlier_fit_half}
% \end{figure}




==> equivalents.tex <==
%auto-ignore
\section{Invariant equivalents}
\cite{unterberger2019global} gives the following integro-differential equation relating the equilibrium measure $\mu_{\infty}$ to the potential $V$ of invariant ensembles: \begin{align}\label{eq:v_stieljtes}
    \frac{\beta}{2}\dashint\frac{1}{x-y}d\mu_{\infty}(y) = V'(x).
\end{align} 
So in the case of real symmetric matrices we have \begin{align}\label{eq:muinf_V_relation}
    \frac{1}{2} G_{\infty}(x) = V'(x)
\end{align}
where $G_{\infty}$ is the Stieljtes transform of $\mu_{\infty}$.

Let $H_N(u)$ be a family of random matrix ensembles defined as in Theorem $4.5$ of \cite{arous2021exponential}, where the parameter $u\in\mathbb{R}^m$. In particular, $\hat{\mu}_{H_N}$ is defined to be the empirical spectral measure of $H_N(u)$ (dependence on $u$ in the all measures is omitted from the notation unless particularly necessary). We assume the existence of a deterministic sequence of measures $\mu_N$ such that \begin{align}
    W_1(\mathbb{E}\muhat{H}, \mu_N) \leq N^{-\kappa}
\end{align}
for large enough $N$ uniformly, and $\kappa$ chosen uniformly for $u$ in compact sets. 
There is assumed to be a limiting measure $\muinf$ such that \begin{align}
    W_1(\muinf, \mu_N) \leq N^{-\kappa}.
\end{align}
Superexponential concentration is also assumed: \begin{align}
    \lim_{N\rightarrow\infty} \frac{1}{N\log{N}}\log \left[\sup_{u} \mathbb{P}(d_{BL}(\muhat{H}(u), \muinf(u)) > \varepsilon\right] = -\infty.
\end{align}
Here $W_1$ and $d_{BL}$ are the Wasserstein-1 and bounded-Lipschitz distances on probability measures on $\mathbb{R}$ respectively.


Given a sufficiently nice $\mu_{\infty}$ (\ref{eq:v_stieljtes}) defines $V$ up-to a constant of integration on $\supp(\muinf)$, but $V$ is not determined on $\R\backslash\supp(\muinf)$.


\begin{lem}\label{lemma:V_unique_mu}
    For compactly supported probability measure $\mu_*$ on $\R$ and real potentials $V$, define \begin{align}
        S_V[\mu_*](y) = V(y) - \int d\mu(x) \log|y-x|.
    \end{align}Suppose $S_V[\mu*]$ is constant on $\supp(\mu_*)$ and $S_V[\mu_8](y) \geq S_V[\mu_*])(y_0)$ for all $y_0\in\supp(\mu_*)$ and $y\in\R$. Then $\mu_*$ is the unique minimiser amongst all probability measures $\mu$ on $\R$ of the energy \begin{align}
        \mathcal{E}_V[\mu] = \int d\mu(x) V(x) - \iint_{x< y} d\mu(x)d\mu(y)\log|x-y|.
    \end{align}
\end{lem}
 \begin{proof}
      INSERT JOSEPH'S STUFF HERE.
 \end{proof}
 
\begin{lem}
    Consider a probability measure $\muinf$ on $\R$ with compact support, absolutely continuous with respect to the Lebesgue measure. Then there exists a potential $V:\R\rightarrow\R$ which yields a well-defined invariant distribution on real symmetric and matrices and for which the equilibrium measure is $\muinf$.
\end{lem}
\begin{proof}
    Absolute continuity of $\muinf$ means it admits a density and so $G_{\infty}$ is continuous on the interior of $\supp(\muinf)$. If follows from ODE theory [REFERENCE] that $G_{\infty}$ possesses an anti-derivative on the interior of $\supp(\muinf)$. Thus the condition $S_V[\muinf]=c$ (a constant) on $\supp(\muinf)$ determines $V$ uniquely on $\supp(\muinf)$. Next observe that, for $y\in\R\backslash\supp(\muinf)$ there exists some constant $R>0$ such that $|x-y| \leq R + |y|$ and so $\log|x-y| \leq |y| + R$. Therefore \begin{equation}
        S_V[\mu](y) \geq V(y) - |y| - R.
    \end{equation}
    So the condition $S_V[\mu](y) \geq c$ for $y\in\R\backslash\supp(\muinf)$ can be satisfied by taking $V(y) = (y-y_0)^2 + b$ for some constants $y_0, b$, which we need not record. There is sufficient freedom in $b, y_0$ left to make $V$ continuous on $\R$. Since $V$ is constructed with Gaussian tails, it can certainly be used to defined a legitimate invariant ensemble of real symmetric random matrices. By Lemma \ref{lemma:V_unique_mu}, the $V$ we have constructed has equilibrium measure $\muinf$.
\end{proof}

==> fourier.tex <==
%auto-ignore
\section{Intermediate results on QUE}\label{sec:fourier}
% We begin with a result extending the statement of QUE in Theorem \ref{thm:que_gaussian} to any fixed number of unit vectors.
% \begin{lem}\label{lem:extended_que}
%     Suppose that QUE holds for $\{\vec{u}_i\}_{i=1}^N$ (in the sense of Theorem \ref{thm:que_gaussian}). Then for any fixed positive integers $m$ and $s$ and any polynomial P in $m$ indeterminates there exists an $\epsilon(P, s)>0$ such that \begin{align}
%         \sup_{\substack{\|\vec{q}_1\|, \ldots, \|\vec{q}_s\|=1\\|I|=m}} \left|\E P\left( (N(\vec{q}_j^T\vec{u}_i)^2)_{\substack{i\in I\\ j=1,\ldots s}}\right) - \E P\left( (\mathcal{N}_{ij}^2)_{\substack{i=1,\ldots, m\\ j=1,\ldots, s}}\right)\right| \lesssim N^{-\epsilon}
%     \end{align}
%     where the $\mathcal{N}_{ij}$ are i.i.d. standard Gaussians.
% \end{lem}
% \begin{proof}
%     It is sufficient to prove that for any non-negative integers $l_1, \ldots l_s$ with $\sum_i l_i = l > 0$, there exists an $\epsilon>0$ such that for large enough $N$ 
%     \begin{align}\label{eq:que_with_several_q_suff}
%          \sup_{\substack{\|\vec{q}_1\|, \ldots, \|\vec{q}_s\|=1\\|I|=m}} \left|\E \prod_{t=1}^s\prod_{i\in |I|}(N(\vec{q}_{j_t}^T\vec{u}_i)^{2})^{l_t} - \E\prod_{i=1}^m\prod_{j=1}^s (\mathcal{N}_{ij}^{2l_j})\right| \lesssim N^{-\epsilon}.
%     \end{align}
%     Begin by writing $(N(\vec{q}_{l_t}^T\vec{u}_i)^{2})^{l_t} = \mathcal{N}_{il_t}^{2l_t} + \mathcal{E}_{il_t}(\vec{q}_{l_t})$, where $\mathcal{E}_{il_t}(\vec{q}_{l_t})$ is some error term, which is a random variable and is dependent on $\vec{u}_i$.\footnote{Note that $\mathcal{E}_{il_t}(\vec{q}_{l_t})$ is not necessarily independent from the the standard Gaussian $\mathcal{N}_{il_t}$.} Then \begin{align}
%         \prod_{t=1}^s\prod_{i\in |I|}(N(\vec{q}_{j_t}^T\vec{u}_i)^{2})^{l_t} &=   \prod_{t=1}^s\prod_{i\in |I|} \mathcal{N}_{il_t}^{2l_t}\notag\\
%         &+ \sum_{t' = 1}^s \mathcal{E}_{il_t'}(\vec{q}_{l_t'})\prod_{t\neq t'}\prod_{i\in |I|} \mathcal{N}_{il_t}^{2l_t}\notag\\
%         &+ \sum_{i\in |I|} \mathcal{E}_{i'l_t}(\vec{q}_{l_t})\prod_{t=1}^s\prod_{i\in |I|/\{i'\}} \mathcal{N}_{il_t}^{2l_t}\notag\\
%         &+ \ldots\label{eq:que_with_several_q_error}
%     \end{align}
%     where the ellipsis represents a fixed (i.e. $N$ independent) number of terms of higher order in the error terms.
%     The triangle inequality and H\"{o}lder's inequality gives \begin{align}
%         \left|\E \sum_{t' = 1}^s \mathcal{E}_{il_t'}(\vec{q}_{l_t'})\prod_{t\neq t'}\prod_{i\in |I|} \mathcal{N}_{il_t}^{2l_t}\right| &\leq \sum_{t'=1}^s \left(\prod_{t\neq t'}\prod_{i\in |I|} \E |\mathcal{E}_{il_t'}(\vec{q}_{l_t'})|^{ms}\E |\mathcal{N}_{il_t}^{2l_t}|^{ms}\right)^{\frac{1}{ms}}\notag
%     \end{align}
%     but then applications of QUE to each of the terms  $\E |\mathcal{E}_{il_t'}(\vec{q}_{l_t'})|^{ms}$ gives some $\epsilon'>0$ such that for large enough $N$
%     \begin{align}
%         \left|\E \sum_{t' = 1}^s \mathcal{E}_{il_t'}(\vec{q}_{l_t'})\prod_{t\neq t'}\prod_{i\in |I|} \mathcal{N}_{il_t}^{2l_t}\right| &\lesssim \sum_{t'=1}^s \left(N^{-\epsilon'}\right)^{\frac{1}{ms}}\lesssim N^{-\epsilon''}
%     \end{align}
%     where the Gaussian moments have been absorbed into the constant factor, and $\epsilon'' = \frac{\epsilon'}{ms}$. Applying the same strategy to all of the error terms in (\ref{eq:que_with_several_q_error}) results in (\ref{eq:que_with_several_q_suff}) as required.
% \end{proof}
This section establishes some intermediate results that follow from assuming QUE for the eigenvectors of a matrix. They will be crucial for our application in the following section. 

\begin{lem}\label{lem:que_preserved_under_rotation}
    Consider a real orthogonal $N\times N$ matrix $U$ with rows $\{\vec{u}_i^T\}_{i=1}^N$. Assume that $\{\vec{u}_i\}_{i=1}^N$ are the eigenvectors of a real random symmetric matrix with QUE. Let $P$ be a fixed $N\times N$ real orthogonal matrix. Let $V = UP$ and denote the rows of $V$ by $\{\vec{v}_i^T\}_{i=1}^N$. Then $\{\vec{v}_i\}_{i=1}^N$ also satisfy QUE.
\end{lem}
\begin{proof}
   Take any unit vector $\vec{q}$, then for any $k=1,\ldots, N$
   \begin{align*}
       \vec{q}^T \vec{v}_k = \sum_{j}q_jV_{kj} &= \sum_{j, l}q_j U_{kl}P_{lj} = (P\vec{q})^T \vec{u}_k.
   \end{align*}
   But $\|P\vec{q}\|_2=\|\vec{q}\|_2=1$ since $P$ is orthogonal, so the statement of QUE for $\{\vec{u}_i\}_{i=1}^N$   transfers directly to $\{\vec{v}_i\}_{i=1}^N$ thanks to the supremum of all unit $\vec{q}$.
\end{proof}

\begin{lem}\label{lem:weaker_col_que}
    Consider a real orthogonal $N\times N$ matrix $U$ with rows $\{\vec{u}_i^T\}_{i=1}^N$. Assume that $\{\vec{u}_i\}_{i=1}^N$ are the eigenvectors of a real random symmetric matrix with QUE. Let $\ell_0(\vec{q}) = \sum_i \1\{q_i \neq 0\}$ count the non-zero elements of a vector with respect to a fixed orthonormal basis $\{\vec{e}_i\}_{i=1}^N$. 
    For any fixed integer $s>0$, define the set \begin{align}
            \Vs = \left\{\vec{q}\in \R^N \mid \|\vec{q}\|=1, ~ \ell_0(\vec{q})=s, ~ q_i=0 ~\forall i\in \TN^c\right\}.
    \end{align}
    Then the columns $\{\vec{u}_i'\}_{i=1}^N$ of $U$ satisfy a weaker form of QUE (for any fixed $n, s>0$):
    \begin{align}\label{eq:que_weak_def}
    \sup_{\substack{\vec{q}\in\Vs \\ }}\sup_{\substack{I \subset \TN\\ |I| = n}} \left|\E P\left(\left(N|\vec{q}^T\vec{u}_k|^2\right)_{k\in I}\right) - \E P\left(\left(|\mathcal{N}_j|^2\right)_{j=1}^m
    \right)\right| \leq N^{-\epsilon}.
\end{align}
We will denote this form of QUE as $\hQUE$.
\end{lem}
\begin{proof}
   Take some $\vec{q}\in \Vs$. Then there exists some $J\subset\TN$ with $|J|=s$ and non-zero $\{q_k\}_{k\in J}$ such that\begin{align*}
       \vec{q}^T\vec{u}_k' = \sum_{j\in J} q_j \vec{e}_j^T \vec{u}_k'.
   \end{align*}
   Take $\{\vec{e}_i\}_{i=1}^N$ to be a standard basis with $(\vec{e}_i)_j = \delta_{ij}$, then $\vec{e}_j^T \vec{u}_k' = U_{jk} = \vec{e}_k^T\vec{u}_j$ so \begin{align*}
       \vec{q}^T\vec{u}_k' = \sum_{j\in J} q_j \vec{e}_k^T\vec{u}_j
   \end{align*}
   but then the coefficients $q_j$ can be absorbed into the definition of the general polynomial in the statement (\ref{eq:que_def}) of QUE for $\{\vec{u}_i\}_{i=1}^N$, which completes the proof, noting that the sum only includes indices contained in $\TN$ owing to the definition of $\Vs$.
\end{proof}

\begin{lem}\label{lem:explicit_error}
    Fix some real numbers $\{y_i\}_{i=1}^r$. Fix also a diagonal matrix $\Lambda$ and an orthonormal set of vectors $\{\vec{v}_i\}_{i=1}^N$ that satisfies $\hQUE$. Then there exists an $\epsilon>0$ and $\vec{\eta}_i\in\C^N$ with
      \begin{align}
       \eta_{ij}^2 &\in [-1, 1] ~ \forall j\in\TN,\\
       \eta_{ij}^2 &\in [-N^{\epsilon}, N^{\epsilon}] ~ \forall j\in\TN^c.\\
   \end{align}
 such that for any integer $l>0$\begin{align}\label{eq:explicit_error_lem1}
        \mathbb{E} \left(\sum_{i=1}^r y_i \vec{v}_i^T\Lambda \vec{v}_i\right)^l - \mathbb{E}\left(\sum_{i=1}^r y_i \frac{1}{N}\vec{g}_i^T\Lambda \vec{g}_i\right)^l = N^{-(1+\epsilon)l} \left( \sum_{i=1}^r y_i \vec{\eta}_i^T\Lambda \vec{\eta}_i\right)^l
    \end{align}
    where the $\vec{g}_i$ are i.i.d. Gaussians $N(0, I_N)$. 
    % Moreover 
    % \begin{align}\label{eq:explicit_error_lem2}
    %     \left| \mathbb{E} \exp\left(i\sum_{i=1}^r y_i \vec{v}_i^T\Lambda \vec{v}_i\right) - \mathbb{E}\exp\left(i\sum_{i=1}^r y_i \frac{1}{N}\vec{g}_i^T\Lambda \vec{g}_i\right)\right| \leq N^{-(1+\epsilon)}\left(\Tr |Y| \Tr |\Lambda|\right) e^{N^{-(1+\epsilon)}\Tr |Y| \Tr |\Lambda|}.
    % \end{align}
\end{lem}
\begin{proof}
   Let $\{\vec{e}_i\}_{i=1}^N$ be the standard orthonormal basis from above. Then 
   \begin{align}
       \E \left(\sum_{i=1}^r y_i \vec{v}_i^T\Lambda \vec{v}_i\right)^l &= \E \sum_{i_1,\ldots, i_l=1}^r\prod_{k=1}^{l} y_{i_k} \vec{v}_{i_k}^T\Lambda\vec{v}_{i_k}\notag\\
       &= \E \sum_{i_1,\ldots, i_l=1}^r\sum_{j_1,\ldots, j_l=1}^N\prod_{k=1}^{l} y_{i_k} \lambda_{j_k} (\vec{e}_{j_k}^T\vec{v}_{i_k})^2\label{eq:que_error_bound1}\\
       \implies \E \left(\sum_{i=1}^r y_i \vec{v}_i^T\Lambda \vec{v}_i\right)^l-\mathbb{E}\left(\sum_{i=1}^r y_i \frac{1}{N}\vec{g}_i^T\Lambda \vec{g}_i\right)^l &= N^{-l}\sum_{i_1,\ldots, i_l=1}^r\sum_{j_1,\ldots, j_l=1}^N\prod_{k=1}^{l} y_{i_k} \lambda_{j_k} \left[N\E(\vec{e}_{j_k}^T\vec{v}_{i_k})^2 - \E (\vec{e}_{j_k}^T\vec{g}_{i_k})^2\right]\notag\\
       &=N^{-l}\sum_{i_1,\ldots, i_l=1}^r\sum_{j_1,\ldots, j_l\in\TN}\prod_{k=1}^{l} y_{i_k} \lambda_{j_k} \left[N\E(\vec{e}_{j_k}^T\vec{v}_{i_k})^2 - \E (\vec{e}_{j_k}^T\vec{g}_{i_k})^2\right]\notag\\
       &+ N^{-l}\sum_{i_1,\ldots, i_l=1}^r\sum_{\substack{j_1\in\TN^c,\\ j_2,\ldots, j_l\in\TN}}\prod_{k=1}^{l} y_{i_k} \lambda_{j_k} \left[N\E(\vec{e}_{j_k}^T\vec{v}_{i_k})^2 - \E (\vec{e}_{j_k}^T\vec{g}_{i_k})^2\right]\notag\\
       &+ \ldots
   \end{align}
   The ellipsis represents the similar terms where further of the $j_1, \ldots, j_r$ are in $\TN^c$.
   For $j\in\TN^c$ the terms \begin{align}
       \left[N\E(\vec{e}_{j_k}^T\vec{v}_{i_k})^2 -\E (\vec{e}_{j_k}^T\vec{g}_{i_k})^2\right]
   \end{align}
   are excluded from the statement of $\hQUE$, however we can still bound them crudely.
   Indeed \begin{align}
       \sum_{j\in\TN^c} N(\vec{e}_j^T\vec{v}_i)^2 = \sum_{j=1}^N N(\vec{e}_j^T\vec{v}_i)^2 - \sum_{j\in\TN}N(\vec{e}_j^T\vec{v}_i)^2 = N - \sum_{j\in\TN}N(\vec{e}_j^T\vec{v}_i)^2
   \end{align}
   but since the bound of $\hQUE$ applies for $j\in\TN$ \begin{align}
       N\E (\vec{e}_j^T\vec{v}_i)^2 = \E(\vec{e}_j^T\vec{g})^2 + o(1) = 1 + o(1) ~~ \forall j\in\TN,
   \end{align}
   then \begin{align}
       \sum_{j\in\TN^c} N(\vec{e}_j^T\vec{v}_i)^2 = N - N(1 + o(1)) = o(N) ~ \implies ~  \E(\vec{e}_j^T\vec{v}_i)^2 = o(1) ~ \forall j \in\TN^c.
   \end{align}
   Note that this is error term is surely far from optimal, but is sufficient here.
   Overall we can now say \begin{align}
      \left|\left[N\E(\vec{e}_{j}^T\vec{v}_{i})^2 -\E (\vec{e}_{j}^T\vec{g}_{i})^2\right]\right| \leq 1 + o(1) \leq 2 ~ \forall j \in\TN^c.
   \end{align}
%   Now 
   
%  \begin{align}
%         \E \left(\sum_{i=1}^r y_i \vec{v}_i^T\Lambda \vec{v}_i\right)^l-\mathbb{E}\left(\sum_{i=1}^r y_i \frac{1}{N}\vec{g}_i^T\Lambda \vec{g}_i\right)^l &= (1 + o(1))N^{-l}\sum_{i_1,\ldots, i_l=1}^r\sum_{j_1,\ldots, j_l\in \TN}\prod_{k=1}^{l} y_{i_k} \lambda_{j_k} \left[N\E(\vec{e}_{j_k}^T\vec{v}_{i_k})^2 - \E (\vec{e}_{j_k}^T\vec{g}_{i_k})^2\right].
%   \end{align}
   We can apply $\hQUE$ to the terms in square parentheses to give $\epsilon_{1}, \ldots, \epsilon_{r}>0$ such that 
   \begin{align}
       |N\E(\vec{e}_{j_k}^T\vec{v}_{i_k})^2 - \E (\vec{e}_{j_k}^T\vec{g}_{i_k})^2| \leq N^{-\epsilon_{i_k}} ~~~ \forall j_k\in\TN ~\forall i_k=1,\ldots, r.
   \end{align}
   We can obtain a single error bound by setting $\epsilon = \min_i \epsilon_i$, where clearly $\epsilon > 0$ and then write
   \begin{align}\label{eq:eta_defn}
    N\E(\vec{e}_{j_k}^T\vec{v}_{i_k})^2 - \E (\vec{e}_{j_k}^T\vec{g}_{i_k})^2 = \eta_{i_kj_k}^2 N^{-\epsilon}    
   \end{align}
   where $ \eta_{i_kj_k}^2 \in [-1, 1]$. To further include the indices $j\in\TN^c$, we extended the expression (\ref{eq:eta_defn}) to all $j_k$ by saying
   \begin{align}
       \eta_{i_kj_k}^2 &\in [-1, 1] ~ \forall j_k\in\TN,\\
       \eta_{i_kj_k}^2 &\in [-N^{\epsilon}, N^{\epsilon}] ~ \forall j_k\in\TN^c.\\
   \end{align}
Overall we have \begin{align}
     \E \left(\sum_{i=1}^r y_i \vec{v}_i^T\Lambda \vec{v}_i\right)^l-\mathbb{E}\left(\sum_{i=1}^r y_i \frac{1}{N}\vec{g}_i^T\Lambda \vec{g}_i\right)^l = N^{-l(1+\epsilon)}\sum_{i_1,\ldots, i_l=1}^r\sum_{j_1,\ldots, j_l=1}^N\prod_{k=1}^{l} y_{i_k} \lambda_{j_k} \eta_{i_kj_k}^2
\end{align}
but by comparing with (\ref{eq:que_error_bound1}) we can rewrite as
\begin{align}
    \E \left(\sum_{i=1}^r y_i \vec{v}_i^T\Lambda \vec{v}_i\right)^l-\mathbb{E}\left(\sum_{i=1}^r y_i \frac{1}{N}\vec{g}_i^T\Lambda \vec{g}_i\right)^l = \left( \sum_{i=1}^r N^{-(1+\epsilon)}y_i \vec{\eta}_i^T\Lambda \vec{\eta}_i\right)^l
\end{align}
where $\vec{\eta}_i^T = (\eta_{i1},\ldots, \eta_{iN})$.

%   \begin{align}
% \left|\E \left(\sum_{i=1}^r y_i \vec{v}_i^T\Lambda \vec{v}_i\right)^l-\mathbb{E}\left(\sum_{i=1}^r y_i \frac{1}{N}\vec{g}_i^T\Lambda \vec{g}_i\right)^l\right| &\leq N^{-l}\sum_{i_1,\ldots, i_l=1}^r\sum_{i_l,\ldots, j_l=1}^N\prod_{k=1}^{l} |y_{i_k}| |\lambda_{j_k}| N^{-\epsilon}\notag\\
% &= N^{-(1+\epsilon)l}\sum_{i_1,\ldots, i_l=1}^r\sum_{i_l,\ldots, j_l=1}^N\prod_{k=1}^{l} |y_{i_k}| |\lambda_{j_k}|.\label{eq:que_error_bound2}
%   \end{align}
%   Comparing (\ref{eq:que_error_bound1}) and (\ref{eq:que_error_bound2}) we see that \begin{align*}
%       \sum_{i_1,\ldots, i_l=1}^r\sum_{i_l,\ldots, j_l=1}^N\prod_{k=1}^{l} |y_{i_k}| |\lambda_{j_k}| =  \left(\sum_{i=1}^r |y_i| \bm{1}^T|\Lambda| \bm{1}\right)^l = \left(\Tr|A|\Tr|\Lambda|\right)^l
%   \end{align*}
%   where $\bm{1} = (1, 1,\ldots, 1)$. This completes the proof of (\ref{eq:explicit_error_lem1}). (\ref{eq:explicit_error_lem2}) follows immediately by writing the exponential as its power series, using its infinite radius of convergence to exchange absolute values, infinite sums and expectations and finally re-summing the error from (\ref{eq:explicit_error_lem1}).
\end{proof}

% \begin{thm}\label{thm:phik_sym_thm}
%     Let $X$ be an $N\times N$ real symmetric random matrix and denote by $\hat{\mu}_N$ its empirical spectral measure. For symmetric matrices $K$ define \begin{align}
%         \Phi(K) = \E_X e^{i\Tr XK}.
%     \end{align}
%     Assume $X$ satisfies the following:
%     \begin{enumerate}
%         \item there exists a deterministic probability measure $\mu_{\infty}$ such that \begin{align*}
%             \lim_{N\rightarrow\infty} \frac{1}{N \log N}\P\left( d_{BL}(\hat{\mu}_N, \mu_{\infty}) > \epsilon \right) = -\infty;
%         \end{align*}
%         \item $\int d\mu_{\infty}(\lambda) |\lambda| < \infty$;
%         \item $X$ has QUE in the sense (\ref{eq:que_def});
%         \item $\Phi(K)$ exists for all symmetric $K$.
%     \end{enumerate}
%     Define a new ensemble $\bar{X} = O^T\Lambda O$ where $O$ is a Haar distributed orthogonal matrix and $\Lambda$ is equal in distribution to the eigenvalues of $X$. Let $\bar{\Phi}$ be the corresponding characteristic function for $\bar{X}$.
%     Suppose that $K = P^TYP$ for some diagonal $Y=\diag(y_1, \ldots, y_r, 0, \ldots, 0)$ and orthogonal $P$, where $r>0$ is fixed and all $y_i\in\R$.
%     Then there exist constants $a, b,\epsilon>0$ such that for large enough $N$ and any symmetric $K$
%     \begin{align}\label{eq:phik_sym_thm1}
%         \left| \Phi(K) - \bar{\Phi}(K)\right| \leq a N^{-\epsilon} \Tr|Y| e^{bN^{-\epsilon}\Tr|Y|}.
%     \end{align}
%     Moreover
%     \begin{align}\label{eq:phik_sym_thm2}
%         \left| \Phi(K) - \Phi(Y)\right| \leq 2a N^{-\epsilon} \Tr|Y| e^{bN^{-\epsilon}\Tr|Y|}.
%     \end{align}
% \end{thm}

% \begin{proof}
%     We begin by writing $X=U^T\lambda U$ where the rows of $U$ are the eigenvectors of $X$ and $\Lambda$ is a diagonal matrix of its eigenvalues. Then \begin{align*}
%         \Phi(K) = \EL \EUL \exp\left(i \Tr U^T\Lambda U P^T Y P\right)=\EL \EUL \exp\left(i \Tr Y(UP^T)^T\Lambda UP^T \right) = \EL \EV \exp\left(i \Tr YV^T\Lambda V\right)
%     \end{align*}
%     where we have defined $V = UP^T \mid \Lambda$. By Lemma \ref{lem:que_preserved_under_rotation} the rows of $V$ have full QUE and thence by Lemma \ref{lem:weaker_col_que} the columns of $V$ satisfy the weakened QUE (\ref{eq:que_weak_def}). Let $\{\vec{v}_i\}_{i=1}^N$ denote the columns of $V$, then \begin{align*}
%         \Phi(K) = \EL \EV \exp\left(i\sum_{j=1}^r y_j \vec{v}_j^T\Lambda \vec{v}_j\right).
%     \end{align*} We can now apply Lemma \ref{lem:explicit_error} to $\Phi(K)$. We can also apply it similarly to $\bar{\Phi}(K)$ because $\bar{X}$ is rotationally invariant and so certainly obeys QUE. Taking $\epsilon$ to be the smaller of the two constants given by the two applications of Lemma (\ref{lem:explicit_error}), we obtain\begin{align*}
%         |\Phi(K) - \bar{\Phi}(K)| &\leq \EL \left[2 N^{-(1+\epsilon)} \left(\Tr |Y| \Tr |\Lambda|\right) e^{N^{-(1+\epsilon)}\Tr|Y| \Tr|\Lambda|}\right]\\
%         &= 2N^{-\epsilon}\Tr|Y|\EL\left[\frac{\Tr |\Lambda|}{N} \exp\left\{N^{-\epsilon}\Tr |Y| \frac{\Tr|\Lambda|}{N}\right\}\right]\\
%           &= 2N^{-\epsilon}\Tr|Y|\EL\left[\int d\hat{\mu}_N(\lambda)|\lambda|\exp\left\{N^{-\epsilon}\Tr |Y| \int d\hat{\mu}_N(\lambda)|\lambda|\right\}\right].
%     \end{align*}
%     We can now apply assumptions 1 and 2 to obtain \begin{align*}
%         |\Phi(K) - \bar{\Phi}(K)| &\leq aN^{-\epsilon}\Tr|Y|\exp\left\{bN^{-\epsilon}\Tr |Y| \right\}
%     \end{align*}
%     for constants $a, b > 0$. This completes the proof of (\ref{eq:phik_sym_thm1}) and (\ref{eq:phik_sym_thm2}) follows immediately: \begin{align*}
%         |\Phi(K) - \Phi(Y)| &\leq |\Phi(K) - \bar{\Phi}(K)| + |\bar{\Phi}(K) - \bar{\Phi}(Y)| + |\bar{\Phi}(Y) - \Phi(Y)| \\
%         & \leq a N^{-\epsilon} \Tr|Y| e^{bN^{-\epsilon}\Tr|Y|} + 0 + a N^{-\epsilon} \Tr|Y| e^{bN^{-\epsilon}\Tr|Y|}.
%     \end{align*}
% \end{proof}

% \begin{rem}
%     The authors of \cite{guhr2006arbitrary,kieburg2009arbitrary} study rotationally invariant random matrix ensembles and demonstrate that the rotational invariance is inherited by the characteristic function. $\Phi(K)$ is central to the supersymmetric method in random matrix theory and symmetries, such as rotational invariance, are essential to achieve the drastic dimensionality reduction which lends the supersymmetric method its power. In Theorem \ref{thm:phik_sym_thm} we have used QUE, a weaker assumption than rotational invariance to obtain a form of approximate rotational invariance of $\Phi$. We believe this result will be independently useful beyond the specific application we pursue in this paper.
% \end{rem}


% \begin{lem}\label{lem:gaussian_moment_approx} Let $\vec{g}_1, \ldots, \vec{g}_r \overset{i.i.d}{\sim} \mathcal{N}(0, I_N)$. Let $\{\vec{u}_i\}_{i=1}^N$ be the normalised eigenvectors of $H_N$ and $\Lambda_N$ its diagonal matrix of eigenvalues. Let $A$ be some real symmetric matrix of rank $r$ with non-zero eigenvalues $\{a_i\}_{i=1}^r$ and let $Q$ be its matrix of orthonormal eigenvectors which we denote by $\{\vec{q}_i\}_{i=1}^N$ (the columns of $Q$). We define $\vec{u}_i^{(Q)} = Q^T\vec{u}_i$ for $i=1,\ldots, N$. For any integer $l\geq 0$, there exists some $\epsilon_l > 0$ and some $N_0
% \in\N$ such that, for all $N\geq N_0$
% \begin{align}
%     \E_{U_N\mid \Lambda_N} \left(\sum_{i=1}^r a_i (\vec{u}_i^{(Q)})^T \Lambda_N \ \vec{u}_i^{(Q)}\right)^l = \E_{\{\vec{g}_i\}_{i=1}^r}  \left(\sum_{i=1}^r a_i \frac{\vec{g}_i^T \Lambda_N \vec{g}_i}{N}\right)^l + \mathcal{O}(1)N^{-\epsilon_l(\{a_i\}_{i=1}^r, \{\lambda_i\}_{i=1}^N)}.
% \end{align}
% Note that $\epsilon_l$ in general depends on the $\{\lambda_i\}$ and $\{a_i\}$ but is positive for any fixed values of both.
% \end{lem}
% \begin{proof}
%     \begin{align}
%         \left(\sum_{i=1}^r a_i (\vec{u}_i^{(Q)})^T \Lambda_N \ \vec{u}_i^{(Q)}\right)^l &= \sum_{i_1, \ldots, i_l=1}^r \prod_{t=1}^l a_{i_t} (\vec{u}_{i_t}^{(Q)})^T\Lambda_N \vec{u}_{i_t}^{(Q)}\notag\\
%         &= \sum_{i_1, \ldots, i_l=1}^r \prod_{t=1}^l a_{i_t} \sum_{j_t=1}^N (\vec{q}_{j_t}^T\vec{u}_{i_t})^2 \lambda_{j_t}\notag\\
%         &= \sum_{i_1, \ldots, i_l=1}^r  \sum_{j_1,\ldots, j_l=1}^N\prod_{t=1}^l a_{i_t}  (\vec{q}_{j_t}^T\vec{u}_{i_t})^2 \lambda_{j_t}\notag\\
%         &=  \sum_{j_1,\ldots, j_l=1}^N\sum_{i_1, \ldots, i_l=1}^r \prod_{t=1}^l a_{i_t}  (\vec{q}_{j_t}^T\vec{u}_{i_t})^2 \lambda_{j_t}\notag
%     \end{align}
%     so \begin{align*}
%         &\left| \E_{U_N\mid \Lambda_N}  \left(\sum_{i=1}^r a_i (\vec{u}_i^{(Q)})^T \Lambda_N  \vec{u}_i^{(Q)}\right)^l - \E_{\{\vec{g}_i\}_{i=1}^r} \left(\sum_{i=1}^r a_i \frac{\vec{g}_i^T \Lambda_N \vec{g}_i}{N}\right)^l \right| \notag\\ 
%         = &N^{-l}  \Bigg| \E_{U_N\mid \Lambda_N} \Bigg(\sum_{i=1}^r a_i  N(\vec{u}_i^{(Q)})^T \Lambda_N  \vec{u}_i^{(Q)}\Bigg)^l - \E_{\{\vec{g}_i\}_{i=1}^r} \Bigg(\sum_{i=1}^r a_i \vec{g}_i^T \Lambda_N \vec{g}_i\Bigg)^l \Bigg|  \\
%         \leq  &N^{-l}\sum_{j_1,\ldots, j_l=1}^N\Bigg|\Bigg(\E_{U_N\mid \Lambda_N} \sum_{i_1, \ldots, i_l=1}^r\prod_{t=1}^l a_{i_t} N (\vec{q}_{j_t}^T\vec{u}_{i_t})^2 \lambda_{j_t}- \E_{\{\vec{g}_i\}_{i=1}^r}\sum_{i_1, \ldots, i_l=1}^r \prod_{t=1}^l a_{i_t}  g_{i_tj_t}^2\lambda_{j_t}\Bigg)\Bigg|.
%     \end{align*}
% Now Lemma \ref{lem:extended_que} can be applied to give 
% \begin{align}
%     \left| \E_{U_N\mid \Lambda_N}  \left(\sum_{i=1}^r a_i (\vec{u}_i^{(Q)})^T \Lambda_N  \vec{u}_i^{(Q)}\right)^l - \E_{\{\vec{g}_i\}_{i=1}^r} \left(\sum_{i=1}^r a_i
%     \frac{\vec{g}_i^T \Lambda_N \vec{g}_i}{N}\right)^l \right|  
%     & \lesssim N^{-l}\sum_{j_1=1,\ldots, j_l=1}^N N^{-\epsilon(\{a_i\}_{i=1}^r, \{\lambda_i\}_{i=1}^N)} = N^{-\epsilon(\{a_i\}_{i=1}^r, \{\lambda_i\}_{i=1}^N)}
%     \end{align}
%     where we have intentionally maintained dependence on the eigenvalues $\Lambda_N$ and of $A$ in the exponents. This completes the proof, noting that $\epsilon$ is in principle dependent on $l$.
% \end{proof}


% \begin{lem}\label{lem:cf_conv}
% Let $X_N$ be a sequence of real random variables for which $|\E X_N^l - \E X^l| \lesssim N^{-\epsilon_l}$ for some $\epsilon_l >0$. Then there exists some $\epsilon>0$ such that  $|\E e^{iX_N} - \E e^{iX}| \lesssim N^{-\epsilon}$.
% \end{lem}
% \begin{proof}
%   We have \begin{align*}
%       e^{iX_N} - e^{iX} = \sum_{k=0}^{K} \frac{i^k}{k!} (X_N^k X^k) + R_K(X_N) - R_K(X)
%   \end{align*}
%   where $R_K(x) = e^{ix} - \sum_{k=0}^{K} \frac{i^kx^k}{k!}$. We have the bound \begin{align*}
%       |R_K(x)| \leq \frac{|x|^{K+1}}{(K+1)!}
%   \end{align*}
%   and so \begin{align*}
%       |\E e^{iX_N} - \E e^{iX}| \leq \frac{|x|^{K+1}}{(K+1)!}
%   \end{align*}
%   THIS NEEDS FINISHING
% \end{proof}

% We now need to take the eigenvalue average. Indeed, \begin{align*}
%     \left|\E e^{-i\Tr AX} -  \E_{\Lambda_N}E_{\{\vec{g}_i\}_{i=1}^r} \exp\left\{-i \sum_{i=1}^r a_i \frac{\vec{g}_i^T \Lambda_N\vec{g}_i}{N}\right\} \right|&\leq \E_{\Lambda_N} N^{-\epsilon(\Lambda_N, \{a_i\})}\\
%     &\leq \E_{\Lambda_N} N^{-\epsilon(\Lambda_N, \{a_i\})}\1\{L \leq \lambda_i \leq U ~ \forall ~i\} + \P(\max_i \lambda_i \geq U)+\P(\min_i \lambda_i \leq L).
% \end{align*}
% Let's take $R$ greater than the right edge of the support of $\mu_{\infty}$ (the limiting measure of $X$) and $L$ less than the left edge of the support. We assume that the support is finite and we further assume no outliers for $X$ in the sense that there exist $\delta_1, \delta_2 > 0$ such that for large enough $N$ \begin{align}
%     \P(\max_i \lambda_i \geq U) \leq N^{-\delta_1}, ~~ \P(\min_i \lambda_i \leq L) \leq N^{-\delta_2}.
% \end{align}
% Then we have \begin{align*}
%     \left|\E e^{-i\Tr AX} -  \E_{\Lambda_N}E_{\{\vec{g}_i\}_{i=1}^r} \exp\left\{-i \sum_{i=1}^r a_i \frac{\vec{g}_i^T \Lambda_N\vec{g}_i}{N}\right\} \right|\leq N^{-\epsilon_{(L, U)}(\{a_i\})} + N^{-\delta_1} + N^{-\delta_2} \lesssim N^{-\delta(\{a_i\}_i}
% \end{align*}
% for some $\delta > 0$ which in principle can depend on the $\{a_i\}$.



















% VERY OLD
% We now have all the ingredients to compute the matrix Fourier transforms required for the remainder of the calculation. Firstly 
% \begin{align*}
%     \Tr H_NA &= \Tr\left[ \diag(\vec{a})(Q^TU_N)\Lambda_N (Q^TU_N)^T\right]\\
%     &= \sum_{i=1}a_i (\vec{u}^{(Q)}_i)^T \Lambda_N \vec{u}^{(Q)}_i
% \end{align*}
% and so Lemma \ref{lem:gaussian_moment_approx} and Lemma \ref{lem:cf_conv} give 
% \begin{align}\label{eq:eigenvector_fourier}
%     \E_{U_N\mid \Lambda_N} e^{-i\Tr H_NA} = \E_{\{\vec{g}_i\}_{i=1}^r} \exp\left\{-i \sum_{i=1}^r a_i \frac{\vec{g}_i^T \Lambda_N\vec{g}_i}{N}\right\} + \|\Lambda_N\|_{\infty}o(1)
% \end{align}
% where the $o(1)$ term is independent of $A$. The Gaussian expectation in (\ref{eq:eigenvector_fourier}) is simple to compute as in \cite{baskerville2021loss}: \begin{align}
%     \int \prod_{j=1}^r \frac{d\vec{g}_j}{(2\pi)^{N/2}}  \exp\left\{-\sum_{i=1}^r\left[  \vec{g}_i^2 + ia_i \frac{\vec{g}_i^T \Lambda_N\vec{g}_i}{N}\right]\right\}
%     &=  \int \prod_{j=1}^r \frac{d\vec{g}_j}{(2\pi)^{N/2}}  \exp\left\{-\sum_{i=1}^r \vec{g}_i^T\left[I_N +  \frac{ia_i \Lambda_N}{N}\right]\vec{g}_i\right\}\notag\\
%     &= \prod_{i=1}^r \det (I + iN^{-1}a_i\Lambda_N)^{-1/2}\notag\\
%     &= \exp\left\{-\frac{1}{2}\sum_{i=1}^r \sum_{j=1}^N \log(1 + iN^{-1}a_i\lambda_j)\right\}.\label{eq:evaluted_gaussian_integral}
% \end{align}


==> notation.tex <==
%auto-ignore
\section{Notation and preliminaries}
\begin{itemize}
    \item For positive integer $N$, we use $[N] = \{1, 2, \ldots, N\}$.
    \item Where necessary for disambiguation, subscripts $N$ on matrices will denote that they are of shape $N\times N$, in particular $I_N$ is the $N\times N$ identity matrix. 
    \item Unless absolutely necessary, we will omit subscripts on $\E$ and leave the distribution implicit. Expectations will either be with respect to i.i.d. Gaussian vectors or the random matrix ensemble $H_N$ unless otherwise indicated.
    \item We'll ultimately work with matrix ensembles $H_N(x)$ for some $x\in\mathbb{R}^m$ as in \cite{arous2021exponential}. In the context of \cite{baskerville2021loss}, $x$ would be a single Gaussian and $H_N(x) = H_N - xI$. The LSD $\mu_{\infty}$ is then a function of $x$ in general, and so the left-edge of its support varies with $x$. As in \cite{arous2021exponential}, we will have some integral $\int_{\mathcal{D}} dx \ldots$ and then asymptotically the integral's principal contribution comes from a subset of $\mathcal{D}$ such that the left edge of the support is non-negative. For now, in the below, we'll just assume that $H_N$'s limiting spectral density ($\mu_{\infty}$) is supported on $[0, \infty)$.
\end{itemize}

==> susy.tex <==
%auto-ignore
\section{Supersymmetric calculation of random determinants}
We begin with a supersymmetric representation for $|\det H_N|$ as found in  \cite{fyodorov2004complexity, fyodorov2005counting, baskerville2021loss} 
    \begin{align}
        |\det H_N| = \limeps \susyint e^{-i\Tr AH_N}
    \end{align}
        where $d\Psi = d\vec{x}_1d\vec{x}_2d\zeta_1d\zeta_1^*d\zeta_2d\zeta_2^*$, $f_N$ is a function which we need not write down and $A = \Amatrix$. Subject to technicalities with interchanging limits and integrals, the objects of interest are \begin{align}
            \phi(A) = \E e^{-i\Tr H_NA}, ~~~~~~ \phi_k(A) = \E \left[e^{-i\Tr H_NA}\1_{i(H_N) = k}\right].
        \end{align}
        
In general, the joint eigenvector and eigenvalue density will not factorise. However we can write \begin{align}
    \phi_k(A) = \E \left[e^{-i\Tr H_NA}\1_{i(H_N) = k}\right] = \E_{\Lambda_N}\left[\E_{U_N\mid \Lambda_N} \left[e^{-i\Tr U_N\Lambda_NU_N^TA}\right]\1_{i(\Lambda_N) = k}\right] \equiv 
    \E_{\Lambda_N}\left[\varphi(A; \Lambda_N)\1_{i(\Lambda_N) = k}\right].
\end{align}

In \cite{baskerville2021loss} or in the case of any invariant ensemble, $\varphi$ would be an Haar integral over the orthogonal group of IZHC type. In \cite{baskerville2021loss} the authors use Gaussian approximations for the columns of $O$ with Haar measure and so obtain the leading order term in $\fourierevec$. Provided that such a leading order term can be obtained here, then the calculation of $\phi_k(A)$ can proceed just as in \cite{baskerville2021loss} and then the the complexity can be obtained.

\medskip
We have already computed $\varphi(A; \Lambda_N)$ in Section \ref{sec:fourier}, in particular (\ref{eq:eigenvector_fourier}) and (\ref{eq:evaluted_gaussian_integral}) combine to give \begin{align}
    \varphi(A; \Lambda_N) &= \exp\left\{-\frac{1}{2}\sum_{i=1}^r \sum_{j=1}^N \log(1 + iN^{-1}a_i\lambda_j)\right\} + \|\Lambda_N\|_{\infty}o(1).\label{eq:varphi_expr}
\end{align}
In particular we have shown that 
\begin{align}\label{eq:phi_k_haar_equivalent}
    \E_{\Lambda_N}\left[\E_{U_N\mid \Lambda_N} \left[e^{-i\Tr U_N\Lambda_NU_N^TA}\right]\right] = \E_{\Lambda_N}\left[\E_{U_N \sim \mu_{Haar}} \left[e^{-i\Tr U_N\Lambda_NU_N^TA}\right]\right] + \|\Lambda_N\|_{\infty}o(1).
\end{align}
\paragraph{The eigenvalue integral.}
Using (\ref{eq:varphi_expr})
\begin{align}
    \phi_k(A) = \E_{\Lambda_N}\left[\exp\left\{-\frac{1}{2}\sum_{i=1}^r \sum_{j=1}^N \log(1 + iN^{-1}a_i\lambda_j)\right\} + \|\Lambda_N\|_{\infty}o(1)\right]\1_{i(\Lambda_N) = k}.
\end{align}

% \notag\\
%     &= \int_{-\infty}^0 \prod_{j=1}^k d\lambda_j \int_0^{\infty} \prod_{j=k+1}^N d\lambda_j p(\lambda_1, \ldots, \lambda_N)\exp\left\{-\frac{1}{2}\sum_{i=1}^r \sum_{j=1}^N \log(1 + iN^{-1}a_i\lambda_j)\right\} ( 1 + o(1) \|A\|_{\infty})
But now consider a new metrix ensemble $J_N \overset{d}{=} O^T \Lambda_N O$ where $\Lambda_N$ is a diagonal matrix of eigenvalues equal in distribution to the eigenvalues of the original matrix ensemble $H_N$, and $O$ is a Haar distributed orthogonal matrix. Let $\psi_k(A) = \E_{J_N} e^{-i\Tr J_NA}$. Then following precisely the procedure in \cite{baskerville2021loss} (i.e. using i.i.d. Gaussian approximations to a fixed number of the columns of $O$) results in \begin{align}
    \psi_k(A) = \E_{\Lambda_N }\left[\exp\left\{-\frac{1}{2}\sum_{i=1}^r \sum_{j=1}^N \log(1 + iN^{-1}a_i\lambda_j)\right\} + \|\Lambda_N\|_{\infty}o(1)\right]\1_{i(\Lambda_N) = k}.
\end{align}



\draft{If this were an invariant ensemble, we could now proceed as in \cite{baskerville2021loss} because the density would factorise, apart from the Vandermonde, which we can deal with. I think we will now need to use the local law again somehow to factorise the density approximately. Expressions like (5.1) in \cite{erdos2017dynamical} might be useful? The assumed local law should should lead to these universality results, but note that those are in the bulk which could be an issue?}


% \section{Index specific complexity of invariant ensembles}
% The objective of this section is to compute $\E |\det J_N| \1_{i(J_N) = k}$ where $J_N$ is a real symmetric $N\times N$ matrix with density proportional to $e^{-\frac{N}{2}\Tr V(J_N)}$, so it's eigenvalues have the law \begin{align}
%     P^N_{V}(\lambda_1, \ldots, \lambda_N) = (Z^N_V)^{-1} |\Delta(\{\lambda_i\}_{i=1}^N)| \prod_{i=1}^N e^{-NV(\lambda_i)}d\lambda_i.
% \end{align}

% We will in fact only be concerned with the annealed limit\begin{align}
%     \lim_{N\rightarrow\infty} \frac{1}{N} \log \E \left[|\det J_N| \1_{i(J_N) = k}\right].
% \end{align}

% We recall important results on large deviations for invariant ensembles.

% \begin{thm}[Theorem 2.6.6 \cite{anderson2010introduction}]
%     Let $(\lambda_1, \ldots, \lambda_N)$ be distributed according to the law $P^N_V$. Let $\mu_V$ be the equilibrium measure and define \begin{align}
%         \alpha_V = \limn \frac{1}{N} \log\frac{Z^N_{NV/(N-1)}}{Z^N_V}.
%     \end{align}
%     Then the bottom eigenvalue satisfies an LDP in $\R$ with speed $N$ and good rate function \begin{align}
%         J_V(x) = \begin{cases}
%                 -\int \log|x-y| d\mu_V(y) + V(x) - \alpha_V ~ &\text{if } x\geq x^*,\\
%                 \infty &\text{otherwise}.
%               \end{cases}
%     \end{align}
% \end{thm}

% \begin{thm}\label{thm:complexity_invariant_index_k}
%     For an invariant ensemble of real symmetric $N\times N$ matrices $J_N$ with potential $V$, let $\mu_V$ be its equilibrium measure. Suppose that $\supp(\mu_V) \cap (-\infty, 0) = \emptyset$, then for $k\geq 0$
%     \begin{align}
%         \limn\frac{1}{N}\log\E\left[|\det J_N|\1_{i(J_N) = k}\right] = \int d\mu_V(\lambda) \log|\lambda| - kJ_V(0).
%     \end{align}
% \end{thm}

% \begin{proof}
%     We begin with a supersymmetric representation for $|\det J_N|$ as found in  \cite{fyodorov2004complexity, fyodorov2005counting, baskerville2021loss} 
%     \begin{align}
%         |\det J_N| = \limeps \susyint e^{-i\Tr AJ_N}
%     \end{align}
%         where $d\Psi = d\vec{x}_1d\vec{x}_2d\zeta_1d\zeta_1^*d\zeta_2d\zeta_2^*$, $f_N$ is a function which we need not write down and $A = \Amatrix$. Subject to technicalities with interchanging limits and integrals, the objects of interest are \begin{align}
%             \phi(A) = \E e^{-i\Tr J_NA}, ~~~~~~ \phi_k(A) = \E \left[e^{-i\Tr J_NA}\1_{i(J_N) = k}\right].
%         \end{align}
%     We then proceed as in \cite{baskerville2021loss}: 
%     \begin{align}
%         \phi_k(A) \propto &\haarint \int_{-\infty}^0 d\lambda_1\ldots d\lambda_k \Delta(\{\lambda_i\}_{i=1}^k) \prod_{i=1}^k e^{-\frac{N}{2}V(\lambda_i)}\notag\\
%         &\int_{0}^{\infty} d\lambda_{k+1}\ldots d\lambda_N \Delta(\{\lambda_i\}_{i=k+1}^N) \prod_{i=k+1}^N e^{-\frac{N}{2}V(\lambda_i)}\notag\\
%         &\exp\left(\sum_{i < k+1 \leq j}|\lambda_i - \lambda_j|\right) e^{-i\Tr O\Lambda O^T A}.
%     \end{align}
% The neglected constant will need tracking in a rigorous proof, but we don't expect it to be troublesome. We can write $\Tr O\Lambda O^T A = \sum_{i=1}^r a_i \vec{o}_i^T\Lambda \vec{o}_i$, where $\vec{o}_i$ are the columns of $O$. We then do the Haar integral using the Gaussian approximation utilised in \cite{baskerville2021loss}. For a rigorous proof, we must write out all of the details, taking care with the error terms etc. For now we will just hand-wave, giving \begin{align}
%      \phi_k(A) \propto &\int_{-\infty}^0 d\lambda_1\ldots d\lambda_k \Delta(\{\lambda_i\}_{i=1}^k) \prod_{i=1}^k e^{-\frac{N}{2}V(\lambda_i)}\notag\\
%             &\int_{0}^{\infty} d\lambda_{k+1}\ldots d\lambda_N \Delta(\{\lambda_i\}_{i=k+1}^N) \prod_{i=k+1}^N e^{-\frac{N}{2}V(\lambda_i)}\notag\\
%             &\exp\left(\sum_{i < k+1 \leq j}|\lambda_i - \lambda_j|\right) \exp\left(-\frac{1}{2}\sum_{i=1}^k\sum_{j=1}^N \log(1 + 2iN^{-1}a_i\lambda_j)\right) + o(1)\notag\\
%             = &\int_{-\infty}^0 d\lambda_1\ldots d\lambda_k \Delta(\{\lambda_i\}_{i=1}^k)\notag\\
%             &\int_{0}^{\infty} d\lambda_{k+1}\ldots d\lambda_N \Delta(\{\lambda_i\}_{i=k+1}^N) \prod_{i=k+1}^N e^{-\frac{N}{2}V(\lambda_i)}\notag\\
%             &\exp\left(N\sum_{i=1}^k\left\{\frac{N-k}{N}\int d\hat{\mu}_{N-k}(\lambda)|\lambda_i - \lambda| - \frac{1}{2}V(\lambda_i)\right\}\right) \exp\left(-\frac{N-k}{2}\sum_{i=1}^k\int d\hat{\mu}_{N-k}(\lambda)\log(1 + 2iN^{-1}a_i\lambda)\right) + o(1).\notag\\
% \end{align}
% We can then use the LDP for $\hat{\mu}_{N-k}$ (speed $N^2$) to justify replacing with $\mu_V$, and we can bound and neglect all the remaining terms (again, this is hand-waving, but all of the details are as in \cite{baskerville2021loss}). This gives \begin{align}
%     \phi_k(A) \propto & e^{-Nk(J_V(0) + o(1))} \exp\left(-\frac{N}{2} \sum_{i=1}^r \int d\mu_V(\lambda) \log(1 + 2iN^{-1}a_i \lambda) + o(N)\right) + o(1).
% \end{align}
% But now consider computing $\phi(A)$ by the same method. One would obtain \begin{align}
%         \phi(A) \propto &\exp\left(-\frac{N}{2} \sum_{i=1}^r \int d\mu_V(\lambda) \log(1 + 2iN^{-1}a_i \lambda) + o(N)\right) + o(1).
% \end{align}
% So then we find \begin{align}
%     \E\left[|\det J_N|\1_{i(J_N) = k}\right] &=  e^{-Nk(J_V(0) + o(1))} \limeps\susyint \exp\left(-\frac{N}{2} \sum_{i=1}^r \int d\mu_V(\lambda) \log(1 + 2iN^{-1}a_i \lambda) + o(N)\right) + o(1)\notag \\
%     &= e^{-Nk(J_V(0) + o(1))}   \exp\left(N\int d\mu_V(\lambda) \log|\lambda| + o(N)\right) + o(1).
% \end{align}
% \end{proof}

% Finally we have obtain as a corollary the result we need.
% \begin{cor}
% For any $\epsilon\in(0,1)$
% \begin{align}
%             \limn\frac{1}{N}\log\E\left[|\det J_N|\1_{i(J_N) < N^{\epsilon}}\right] = \int d\mu_V(\lambda) \log|\lambda|.
% \end{align}

% \end{cor}
% \begin{proof}
%  By Theorem \ref{thm:complexity_invariant_index_k}
%     \begin{align}
%         \E\left[|\det J_N|\1_{i(J_N) < N^{\epsilon}}\right] &= \E\left[|\det J_N|\1_{i(J_N) = 0}\right] +  \sum_{k=1}^{N^{\epsilon}}\E\left[|\det J_N|\1_{i(J_N) = k}\right]\notag\\
%         &\leq \E\left[|\det J_N|\1_{i(J_N) = 0}\right]\left(1 + N^{\epsilon} e^{-NJ_V(0)}\right)
%     \end{align}
%     and clearly \begin{align}
%           \E\left[|\det J_N|\1_{i(J_N) < N^{\epsilon}}\right] \geq \E\left[|\det J_N|\1_{i(J_N) = 0}\right]
%     \end{align}
%     so we are done.
% \end{proof}



